Configuration Balancing for Stochastic Requests

The configuration balancing problem with stochastic requests generalizes many well-studied resource allocation problems such as load balancing and virtual circuit routing. In it, we have $m$ resources and $n$ requests. Each request has multiple possible configurations, each of which increases the load of each resource by some amount. The goal is to select one configuration for each request to minimize the makespan: the load of the most-loaded resource. In our work, we focus on a stochastic setting, where we only know the distribution for how each configuration increases the resource loads, learning the realized value only after a configuration is chosen. We develop both offline and online algorithms for configuration balancing with stochastic requests. When the requests are known offline, we give a non-adaptive policy for configuration balancing with stochastic requests that $O(\frac{\log m}{\log \log m})$-approximates the optimal adaptive policy. In particular, this closes the adaptivity gap for this problem as there is an asymptotically matching lower bound even for the very special case of load balancing on identical machines. When requests arrive online in a list, we give a non-adaptive policy that is $O(\log m)$ competitive. Again, this result is asymptotically tight due to information-theoretic lower bounds for very special cases (e.g., for load balancing on unrelated machines). Finally, we show how to leverage adaptivity in the special case of load balancing on related machines to obtain a constant-factor approximation offline and an $O(\log \log m)$-approximation online. A crucial technical ingredient in all of our results is a new structural characterization of the optimal adaptive policy that allows us to limit the correlations between its decisions.

==> old/old_config_on.tex <==
\section{Online Configuration Balancing}\label{sec_online_config}
In this section, we formally introduce \emph{configuration balancing}\fra{Do we have another name for the problem or to we want to stick with configuration balancing?} and present competitive online algorithms. Configuration balancing is a generalization of virtual circuit routing. We start by considering deterministic requests and show afterwards how to extend our results to stochastic requests if there is a near-optimal solution satisfying mild assumptions. 


\subsection{Deterministic Requests}

In (offline) configuration balancing, there are~$m$ resources given as well as~$n$ requests. Every request~$j$ has~$q_j$ associated load configurations~$x_j(1), \ldots, x_j(q_j) \in \RR_{\geq 0}^m$. For every request, exactly one configuration~$c$ has to be chosen which adds load~$x_j(c)$ to the resources, i.e., load~$x_{ij}(c)$ is added to resource~$i$ for~$i\in [m]$. The goal is to minimize the maximum load,~$\max_i \{ \sum_{j} x_{ij}(c_j) \}$, where~$c_j$ is the configuration chosen for request~$j$. 

Load balancing on unrelated machines can be modelled as a configuration balancing problem by representing the~$m$ choices of how to assign a job to a machine as~$m$ distinct configurations: There are~$m$ resources, every job has~$m$ configurations, and we set~$x_{ij}(c) = p_{ij}$ \fra{What are the parameters for the deterministic problem?} if~$i=c$ and~$x_{ij}(c) = 0$ otherwise. 

Virtual circuit routing can also be interpreted as a configuration balancing problem in the following way. The~$m$ resources represent the~$m$ edges of the graph~$G=(V,E)$, while each possible~$s_j$--$t_j$ path~$P$ is identified with one configuration: We set~$x_{ej}(P) = x_{ej}$ if edge~$e$ is part of path~$P$ and~$x_{ej}(P) = 0$ otherwise. \fra{Check notation for virtual circuit routing.} 

It is natural to consider \emph{online configuration balancing} where the~$n$ requests arrive online one by one, and for each request, one configuration has to be irrevocably selected before the next request appears. In the following, we present an online algorithm for configuration balancing that achieves a competitive ratio of~$O(\log m)$, which is best possible due to the lower bound of~$\Omega(\log m)$ on the competitive ratio of any deterministic algorithm for online load balancing on unrelated machines \cite{DBLP:journals/jal/AzarNR95}. 

The key ingredient is to notice that the classical approach of using a potential function can be generalized to online configuration balancing. Based on minimizing the increase in the potential, the online algorithm is then able to greedily choose the load configuration for request~$j$. Aspnes et al.~\cite{AspnesAFPW97} are the first to employ this approach for online load balancing problems, more precisely for online virtual circuit routing. 

The second ingredient is to observe that online configuration balancing satisfies the conditons of \Cref{lem_guess_and_double}. Hence, we can assume from now on that we have access to a good guess~$\lambda$ on the optimal solution~$\Opt$, and we will design an algorithm that either returns a solution with maximum load at most~$O(\log m) \lambda$ or gives a certificate that~$\Opt$ is as least~$\lambda$. 

Let~$\load_{ij}$ denote the load on resource~$i \in [m]$ \emph{after} the online algorithm chose a configuration for request~$j$. Let~$\phi(\load) = \sum_{i=1}^m (3/2)^{\load_i / \lambda}$ be the potential of load vector~$\load$. 

The algorithm works as follows: Upon arrival of request~$j+1$, we would like to choose the configuration~$c_{j+1} \in [q_{j+1}]$ that minimizes~$\phi(\load_j + x_{j+1}(c)) - \phi(\load_j)$. If indeed~$\load_{ij} + x_{i j+1}(c_{j+1}) \leq O( \log m) \lambda$ holds for all resources~$i$, we assign configuration~$c_{j+1}$ to request~$j+1$ and update the load vector~$\load_{j+1} \leftarrow \load_j + x_{j+1}(c_{j+1})$. If~$\load_{ij} + x_{ij+1} > O(\log m) \lambda$ for some resource~$i$, we return~$\Opt > \lambda$. We summarize the algorithm below.

\begin{algorithm}
    \DontPrintSemicolon
    \caption{Online Configuration Balancing}
    \label{alg_on_config}  
    \textbf{upon arrival of request $j$}\;
    $c_j \leftarrow \arg \min_i \{ \phi(\load + x(c)) - \phi(\load)$\}\;
    \uIf{
    $\load_i + x_{ij}(c_j) \leq O(\log m) \lambda$ for all $i$}{
    choose $c_j$ for $j$ \;
    $\load \leftarrow \load + x_j(c_j)$ \;    }
    \Else{
    fail \;
    }
\end{algorithm}

For analyzing the competitive ratio of this algorithm, we compare its maximum load with the objective function value of the linear program~\eqref{eq_lpconfig}. The variables~$y_{cj}$ represent the fractional extend to which configuration~$c$ is chosen for request~$j\in[n]$, and the first constraint ensures that these fractions sum up to one. The second set of constraints bound the load on resource~$i \in [m]$. This LP clearly is a relaxation of offline configuration balancing, which can be encoded by adding integrality constraints on the~$y_{cj}$ variables to the LP.  

\begin{equation}\tag{$\lpconfig$}\label{eq_lpconfig}
   \begin{array}{rll}
     \sum_{c=1}^{q_j} y_{cj} &  = 1 &\quad\forall~j\in[n] \\
     \sum_{j=1}^n \sum_{c=1}^{q_j} x_{ij}(c) \cdot y_{cj}  &  \leq \lambda &\quad\forall~i\in[m] \\
     y_{cj} & = 0 & \quad \forall~ j \in [n], \forall~c \in [q_j]: \exists~i: x_{ij}(c) > \lambda \\ 
     y_{cj} & \geq 0 & \quad \forall~j\in[n], \forall~c \in [q_j] 
    \end{array} 
\end{equation}

We point out that this LP has an integrality gap of~$\Omega(\log m)$, which follows immediately from the path assignment LP for virtual circuit routing \addref. Hence, a straightforward analysis of \Cref{alg_on_config} using \eqref{eq_lpconfig} yields a competitive factor of~$O(\log^2 m)$, where one factor~$O(\log m)$ is due to the aforementioned integrality gap while the second factor~$O(\log m)$ is due to the use of the potential function. Crucially, the particular choices of \Cref{alg_on_config} allow us to directly compare the algorithm's solution to \emph{any} (not necessarily integral) feasible solution of~\eqref{eq_lpconfig}, implying a tight competitive ratio of~$O(\log m)$. 

\begin{theorem}\label{thm_dcb_on}
    If~\eqref{eq_lpconfig} is feasible for~$\lambda >0$, then \Cref{alg_on_config} guarantees a maximum load $O(\log m)\lambda$.  
\end{theorem}

\begin{proof}
    Let~$(y_{cj}) \in [0,1]$ be a feasible solution to~\eqref{eq_lpconfig}. Since \Cref{alg_on_config} chooses a configuration~$c_j$ minimizing the increase in potential, we have~$\phi(\load_{j-1} + x_j(c_j)) - \phi(\load_{j-1}) \leq \phi(\load_{j-1} + x_j(c)) - \phi(\load_{j-1})$ for all configurations~$c \in [q_j]$. As~$\sum_{c=1}^{q_j} y_{c_j} = 1$ by feasibility of~$(y_{c_j})$, this implies
    \begin{equation}\label{eq_greedy_increase}
        \phi(\load_{j-1} + x_j(c_j)) - \phi(\load_{j-1}) \leq \sum_{c=1}^{q_j} y_{c_j} \phi(\load_{j-1} + x_{j}(c)) - \phi(\load_{j-1}). 
    \end{equation}

    For simplicity, let~$x_{j}$ denote the load vector of configuration~$c_j$. Further, let~$\load_0 = 0 \in \RR^m$ be the all-zero vector. We can now bound the increase in potential incurred by \Cref{alg_on_config} as follows: 
    \begin{align*}
        \phi(\load_n) - \phi(\load_0) 
        & = \sum_{j=1}^n \sum_{i=1}^m \frac32^{\load_{ij-1}/\lambda} \Big( \frac32^{x_{ij}/\lambda} - 1 \Big) \\ 
        & \leq \sum_{j=1}^n \sum_{c=1}^{q_j} y_{c_j} 
            \sum_{i=1}^m  \frac32^{\load_{ij-1}/\lambda} \Big( \frac32^{x_{ij}(c)/\lambda} - 1 \Big) \\ 
       &  \leq 
       \sum_{i=1}^m \frac32^{\load_{in}/\lambda} \sum_{j=1}^n \sum_{c=1}^{q_j} y_{c_j} \Big( \frac32^{x_{ij}(c)/\lambda} -1 \Big), 
   \intertext{where the first inequality holds due to~\eqref{eq_greedy_increase}, and the second inequality holds because the load on machine~$i$ only increases over time. 
       Using a simple algebraic computation, we can bound $\frac32^z - 1 \leq \frac12 z$ for~$z \in [0,1]$. As~$y_{c_j}$ is feasible, we know that~$x_{ij}(c) \leq \lambda$ for all~$c$ with~$y_{c_j} > 0$. Hence, }
        \phi(\load_n) - \phi(\load_0)  & \leq \sum_{i=1}^m \frac32^{\load_{in}/\lambda} \sum_{j=1}^n \sum_{c=1}^{q_j} y_{c_j} \frac{x_{ij}(c)}{2\lambda}
        \intertext{Using again that~$y_{c_j}$ is feasible and satisfies $\sum_{j=1}^n \sum_{c=1}^{q_j} x_{ij}(c) \cdot y_{c_j}  \leq \lambda$ for all resources~$i \in [m]$, we get} 
        \phi(\load_n) - \phi(\load_0) & \leq \frac12 \sum_{i=1}^m \frac32^{\load_{in}/\lambda} = \frac12 \phi(\load_n) 
   \end{align*}
    After rearranging, we get $\phi(\load_n) \leq 2 \phi(\load_0) = 2m$ by choice of~$\load_0$. Taking logarithms and using that~$\log_{3/2}(z)$ is monotonically increasing, we conclude the proof with 
    \begin{equation*}
        \max_{1 \leq i \leq m} \load_{in} \leq \log_{3/2} (2m).
    \end{equation*}
\end{proof}




\subsection{Stochastic Requests}

The goal of this section is to extend \Cref{thm_dcb_on} to stochastic requests. More precisely, every request~$j\in[n]$ is associated with~$q_j$ \emph{random} load configurations~$X_j(1), \ldots, X_j(q_j) \in \RR_{\geq 0}^m$, where~$X_j(c)$ and~$X_{j'}(c')$ are independent if~$j \neq j'$ for~$1\leq c \leq  q_j$ and~$1\leq c' \leq q_{j'}$ . Selecting configuration~$c_j$ for request~$j$ adds the random load~$X_{ij}(c_j)$ to resource~$i$. As in its deterministic counterpart, the task is to select exactly one configuration~$c_j$ for every request~$j$ while minimizing the maximum load over the resources. 

To build on the work of the previous section, we focus on those variants of stochastic configuration balancing, where the random variables can be split into a truncated and an exceptional part without increasing \Opt{} by more than a constant factor. Let~$\tau$ be a fixed threshold. For a random variable~$X$, we recall the definition of the truncated part~$X^T = X \cdot \one_{X < \tau}$ and of the exceptional part~$X^E = X \cdot \one_{X \geq \tau}$. 

The main idea for generalizing \Cref{thm_dcb_on} to the stochastic setting is to treat the exceptional parts of a requests's configuration as a \emph{resource requirement} for an additional, artificial resource indexed by~$0$. To this end, let~$\lambda$ denote the current guess of the optimum, and let~$\tau = 2 \lambda$ be the truncation threshold. Given a request~$j$ and one of its configurations~$c \in [q_j]$, let~$x_{0j}(c) := \EE[\max_{1\leq i \leq m} X_{ij}^E(c)]$ and~$x_{ij}(c) := \EE[X_{ij}^T(c)]$. We interpret~$x(c) \in \RR_{\geq 0}^m$,~$c \in [q_j]$ as input to (deterministic) online configuration balancing with~$m+1$ resources. We summarize the algorithm below.

\begin{algorithm}
    \DontPrintSemicolon
    \caption{Online Configuration Balancing with Stochastic Requests}
    \label{alg_on_stoch_config}  
    \textbf{upon arrival of request $j$}\;
    $x_{0j}(c) \leftarrow \EE[\max_i X_{ij}^E(c)]$ for all $1 \leq c \leq [q_j]$\;
    $x_{ij}(c) \leftarrow \EE[X_{ij}^T(c)]$ for all $c \in [q_j]$ and $i \in [m]$\;
    run \Cref{alg_on_config} for configuration vector~$x_j(c)$ with resources $0,\ldots, m$
\end{algorithm}

For the analysis of the algorithm, we rely on the following generalization of~\eqref{eq_lpconfig}. The variables~$y_{cj}$ denote again the fraction to which configuration~$c$ is selected for request~$j$. 

\begin{equation}\tag{$\lpstochconfig$}\label{eq_lpstochconfig}
   \begin{array}{rll}
     \sum_{c=1}^{q_j} y_{cj} &  = 1 &\quad\forall~j\in[n] \\
     \sum_{j=1}^n \sum_{c=1}^{q_j} \EE[X_{ij}^T(c)] \cdot y_{cj}  &  \leq 2 \lambda &\quad\forall~i\in[m] \\
     \sum_{j=1}^n \sum_{c=1}^{q_j} \EE[\max_i X_{ij}^E(c)] \cdot y_{cj} & \leq 2 \lambda \\
     y_{cj} & = 0 & \quad \forall~ j \in [n], \forall~c \in [q_j]: \exists~i: \EE[X_{ij}(c)] > \lambda \\ 
     y_{cj} & \geq 0 & \quad \forall~j\in[n], \forall~c \in [q_j] 
    \end{array} 
\end{equation}

With the definition of $x_{ij}(c)$ for~$j \in [n]$,~$c \in [q_j]$, and~$0 \leq i \leq m$ used by \Cref{alg_on_stoch_config}, this LP is equivalent to~\eqref{eq_lpconfig}. Hence, \Cref{thm_dcb_on} immediately guarantees $\sum_{j=1}^n \EE[X_{ij}^T(c_j)] \leq O(\log m) \lambda$ for all resources~$i\in [m]$ as well as 
$\sum_{j=1}^n \EE[\max_i X_{ij}^E(c_j)] \cdot y_{cj} \leq O(\log m) \lambda$ 
if~\eqref{eq_lpstochconfig} is feasible for~$\lambda$. In order to extend this to a bound on the maximum load incurred by~\Cref{alg_on_stoch_config}, we need the following bound on the maximum of sums of bounded random variables. 

\begin{lem}\label{lem_max_bound_logm}
    Let~$S_1, \ldots, S_m$ be sums of independent random variables bounded in~$[0,\tau]$ such that~$\EE[S_i] \leq O(\log m) \tau$ for all~$1 \leq i \leq m$. Then,~$\EE[\max_i S_i] \leq O(\log m) \tau$. 
\end{lem}

\begin{proof}
    Let~$C \in \RR$ such that~$\EE[S_i] \leq C \tau \log m$ for all~$1 \leq i \leq m$ and fix~$t > 2e C \tau \log m$, where~$e$ is the Euler constant. Fixing~$i\in[m]$, we know that the random variables constituting~$S_i$ are independent and bounded by~$\tau$. Hence, using the third Chernoff-Hoeffding bound in \Cref{lem_chernoff}, we have~$\PP[S_ i > t] < 2^{-t}$. Therefore, 
    \begin{align*}
        \EE\Big[ \max_{1 \leq i \leq m} S_i \Big] \notag
        & = \int_{0}^\infty \PP\Big[ \max_{1 \leq i \leq m} S_i  > t  \Big] dt \\
        & \leq O(\log m)\tau + \int_{2eC \tau \log m}^\infty  \PP\Big[ \max_{1 \leq i \leq m} S_i  > t  \Big] dt \\
        & \leq O(\log m)\tau + \sum_{i=1}^m \int_{2eC \tau \log m}^\infty \PP\Big[ S_i  > t  \Big] dt \\
        & \leq O(\log m)\tau + m \int_{2 e C \tau \log m}^\infty 2^{-t} dt \\
        & = O(\log m) \tau, 
    \end{align*}
    where the third line uses a union bound over all~$i \in [m]$. 
    
    Note that the proof only requires that the random variables contributing to~$S_i$ for a fixed~$i$ are independent, but it is not necessary, that the~$S_i$ are independent from each other. 
\end{proof}



We are now ready to prove the main result of this section, the following theorem. 

\begin{theorem}\label{thm_cb_on}
    If \eqref{eq_lpstochconfig} is feasible for~$\lambda > 0$, then \Cref{alg_on_stoch_config} achieves a maximum load of~$O(\log m)\lambda$. 
\end{theorem}

\begin{proof}
    As before, let~$c_j$ denote the configuration selected by~\Cref{alg_on_stoch_config} for request~$j$. Then, 
    \[
        \EE \Big[\max_{i \in [m]} \sum_{j=1}^n X_{ij}(c_j) \Big] \leq \EE \Big[\max_{i \in [m]} \sum_{j=1}^n X_{ij}^T(c_j) \Big] + \EE \Big[\max_{i \in [m]} \sum_{j=1}^n X_{ij}^E(c_j) \Big]. 
    \]
    Hence, it is sufficient to bound the exceptional and the truncated parts separately. The correct bound on the truncated parts follows immediately from the fact that~\Cref{thm_dcb_on} guarantees~$\sum_{j=1}^n \EE[X_{ij}^T(c_j)] \leq O(\log m) \lambda$ for all~$i \in [m]$ and \Cref{lem_max_bound_logm}. 
    For the exceptional parts, we observe that 
    \[
        \EE\Big[\max_{i \in [m]} \sum_{j=1}^n X_{ij}^E(c_j) \Big] \leq 
        \EE\Big[\sum_{j=1}^n \max_{i \in [m]} X_{ij}^E(c_j) \Big] \leq O(\log m) \lambda,
    \]
    where the second inequality follows again from~\Cref{thm_dcb_on}. 
\end{proof}

%So far, we haven't discussed whether \Cref{alg_on_config} is always able to find configuration~$c_j$ that minimizes the increase in the potential and dictates the choice for request~$j$. In the setting of load balancing on unrelated machines, there are at most~$m$ configurations possible, which allows for finding the minimizer~$c_j$ efficiently. Hence, we conclude this section with the following proof. 

We are now ready to prove one of our main results, the upper bound on online stochastic load balancing on unrelated machines. 

\begin{proof}[Proof of \Cref{thm_unrel_lb_on}] 
    We reduce online load balancing on unrelated machines to configuration balancing as described in the beginning of this section. That is, for each job~$j$, we create~$m$ configuration vectors by defining
    \begin{equation*}
        X_{ij}(c) =
        \begin{cases}
            X_{ij} & \textup{ if } c = i \\
            0 & \textup{ otherwise.}
        \end{cases} 
    \end{equation*}
    Hence, every job has at most~$m$ configurations associated, which implies that the configuration~$c_j$, that minimizes the increase in the potential function, can be found efficiently. Recall that selecting configuration~$c$ for job~$j$ corresponds to assigning~$j$ to machine~$c$. Further, note that~$\EE[\max_{1 \leq i \leq m} X_{ij}^E(c)] = \EE[X_{cj}^E]$. Hence, by \Cref{lem_gaplp_feasible},~\eqref{eq_lpstochconfig} is feasible. Thus, the conditions of \Cref{thm_cb_on} are satisfied which implies \Cref{thm_unrel_lb_on}. 
\end{proof}


\subsection{Online Load Balancing on Related Machines} 

In this section, we improve upon \Cref{thm_unrel_lb_on} in the special case of online load balancing on related machines, that is, we prove \Cref{thm_rel_lb_on}. Recall that, by \Cref{lem_rel_smooth}, we can assume that the set of machines is smoothed, i.e., there are at most~$m'= O(\log m)$ many groups, where group~$k \in [m']$ consists of~$m_k$ machines with speed~$s_k$ such that~$s_1 < \ldots < s_{m}$. 

We truncate the processing times of jobs at~$\tau = 2 \lambda s_k$, where~$\lambda$ is the current guess of~$\EE[\Opt]$. That is~$X_{kj}^T$ and~$X_{kj}^E$ are defined with respect to~$\tau$. Further, we combine the machines of group~$k$ to one supermachine of processing power~$m_k$, which can be viewed as the \emph{average load} on machines of group~$k$.  That is, the configuration vector~$x_j(c)$ for~$c \in [m']$ is defined by setting~$x_{cj}(c) = \EE\Big[ \frac{X_{cj}^T}{m_c} \Big]$,~$x_{kj}(c) = 0$ if~$k \neq c$ and~$x_{0j}(c) = \EE[X_{cj}^E]$. Afterwards, we run \Cref{alg_on_config} with resources~$0, \ldots, m'$ to obtain the configuration~$c_j$ that minimizes the increase in potential. Given the configuration~$c_j$, we schedule job~$j$ on group~$c_j$ using list scheduling as in \Cref{sec_off_rel}. (Note that in the special case of load balancing, there is a one-to-one correspondence between the set of machines and the possible configurations of a job-request.)

\begin{algorithm}
    \DontPrintSemicolon
    \caption{Online Load Balancing on Related Machines}
    \label{alg_on_stoch_rel}  
    \textbf{upon arrival of request $j$}\;
    $x_{0j}(c) \leftarrow \EE[X_{cj}^E]$ for all $1 \leq c \leq m'$\;
    $x_{kj}(c) \leftarrow \EE[X_{cj}^T/ m_c]$ if $k=c$ for all~$1\leq c, k \leq m'$ \;
    $x_{kj}(c) \leftarrow 0$ if $c\neq k$ for all~$1\leq c, k \leq m'$ \;
    run \Cref{alg_on_config} for configuration vector~$x_j(c)$ with resources $0,\ldots, m'$ \;
    list schedule $j$ on group $c_j$
\end{algorithm}

\begin{theorem}
    If~$\EE[\Opt] \leq \lambda$, \Cref{alg_on_stoch_rel} achieves a maximum load of~$O(\log \log m) \lambda$. 
\end{theorem}

\begin{proof}
    We start by showing that~\eqref{eq_lpconfig} is feasible for the setting of \Cref{alg_on_stoch_rel}, i.e., for the configuration vectors~$x_j(c)$ and the resources defined above. To this end, we consider~\eqref{eq_lpstochconfig} for the original setting, i.e., before aggregating the machines of one group to a supermachine. We use again the reduction of online load balancing to online configuration balancing as in the proof of \Cref{thm_unrel_lb_on}.
    
    By \Cref{lem_gaplp_feasible},~$\EE[\Opt] \leq \lambda$ implies that~\eqref{eq_lpstochconfig} is feasible for~$\lambda$. Aggregating the variables~$y_{cj}$ for all indices~$c$ belonging to group~$k$ to~$y_{kj}'$ and adding the constraints $\sum_{j=1}^n \sum_{c = 1}^{m} \EE[X_{ij}^T(c)] \cdot y_{cj} \leq 2 \lambda$ for all machines~$i$ from group~$k$ implies that 
    \[
        \sum_{j=1}^n \sum_{c' = 1}^{m'} x_{kj}(c') \cdot y_{c'j}' 
        =\sum_{j=1}^n \EE\bigg[\frac{X_{kj}^T}{m_k}\bigg] \cdot y_{kj}' 
        = \frac1{m_k} \sum_{j=1}^n \sum_{i \in \textup{ group } k} \sum_{c=1}^m \EE[X_{ij}^T(c)] y_{cj} 
        \leq 2 \lambda,
    \]
    
    Recall that~$x_{0j}(c) = \EE [X_{cj}^E]$. Thus, 
    \[
        \sum_{j=1}^n \sum_{c' = 1}^{m'} x_{0j}(c') \cdot y_{c'j}' = \sum_{j=1}^n \sum_{c' =1}^{m'} \EE \big[X_{cj}^E\big] y_{c'j}' = \sum_{j=1}^n \sum_{c=1}^m \EE \big[X_{cj}^E\big] y_{cj} \leq 2 \lambda. 
    \]
    Combining these two calculations guarantees that~\eqref{eq_lpconfig} is feasible, which is the condition of \Cref{thm_dcb_on}. Hence, combining \Cref{lem_max_bound_logm} with \Cref{thm_dcb_on} as done in the proof of \Cref{thm_cb_on}, we can conclude that \Cref{alg_on_stoch_rel} achieves an expected maximum load of~$O(\log m') = O(\log \log m)$. 
\end{proof}

\subsection{Online Virtual Circuit Routing}
\fra{talk about how to find the minimizing path}

==> old/old_intro.tex <==
\section{Introduction}\label{sec_intro}

Consider the \emph{load balancing} problem: we wish to schedule $n$ jobs on $m$ machines to minimize the makespan (the load of the most loaded machine.) We are interested in the setting where the job sizes are stochastic. In the most general unrelated machine setting, we assume that the processing time of job $j$ on machine $i$ is a random variable $X_{ij}$ with known distribution such that the $X_{ij}$'s are independent across different jobs $j$. However, the actual realized size of job $j$ is observed only after deciding to schedule job $j$ on some machine. The objective is to minimize the expected makespan, so the quantity:
\[\mathbb{E} \big[\max_i \sum_{j \rightarrow i} X_{ij} \big],\]
where the sum is over all jobs $j$ scheduled on machine $i$. We also study the special case of related machines, where each machine $i$ has a speed $s_i > 0$ and each job has a single size $X_j$ such that $X_{ij} = \frac{X_j}{s_i}$.

In the offline setting, the size distributions of all $n$ jobs are known up-front, and they can be scheduled in any order. In the online setting, the jobs arrive one-by-one such that we learn the size distributions of a job upon its arrival, and we have no knowledge of future arrivals.

In general, we allow the algorithm to make the next scheduling decision using knowledge of the realized sizes of all previously-scheduled jobs. We call such scheduling policies \emph{adaptive}. Conversely, a non-adaptive policy is one that fixes an assignment of jobs to machines without using any knowledge of the realized jobs sizes. The goal of this paper is to approximate the optimal offline adaptive policy.

The second problem we consider is the closely related \emph{\alert{virtual circuit routing} problem} \rud{probably has better name/exposition}\fra{previous papers call it virtual circuit routing}. In this problem, we wish to route $n$ requests through a network (directed graph) on $m$ edges to minimize the makespan (the load of the most loaded edge.) Each request $j$ consists of a source-sink pair $(s_j, t_j)$ such that we must choose a $s_j$--$t_j$ path in the network to route this request. For every edge $e$ along this path, we increase its load by a random size $X_{ej}$ with known distribution such that the $X_{ej}$'s are independent across different jobs $j$. We study the related machines analogue, where each job has a single size $X_j$ and each edge $e$ has a ``speed'' $s_e < 0$ such that $X_{ej} = \frac{X_j}{s_e}$. Again, we are interested in offline- and online algorithms that approximate the optimal offline adaptive policy.

Load balancing is well-studied with deterministic job sizes. If all jobs are known offline, a $2$-approximation is known in the most general unrelated machines setting \cite{DBLP:journals/mp/LenstraST90}. %Further, if jobs arrive one-by-one online, then a there is a $O(1)$-competitive algorithm for related machines and a $O(\log m)$-competitive algorithm for unrelated machines \alert{Cite whatever}.

When job sizes are stochastic, prior work has focused on approximating the optimal \emph{non-adaptive} policy. For identical machines ($X_{ij} = X_j$ for all jobs $j$), there is an algorithm that computes a non-adaptive policy that $O(1)$-approximates the optimal non-adaptive policy \cite{DBLP:journals/siamcomp/KleinbergRT00}. This result was extended to give a $O(1)$-approximation for unrelated machines by \cite{DBLP:journals/mor/Gupta0NS21}.

However, in our work we focus on approximating the stronger optimal \emph{adaptive} policy. It is known that the \emph{adaptivity gap} (the maximum ratio between the expected makespan of the optimal adaptive- and non-adaptive policies) is $\Omega(\frac{\log m}{\log \log m})$ even for the simplest case of identical machines \cite{DBLP:journals/mor/Gupta0NS21}. Thus, previous work on approximating the optimal non-adaptive policy does not immediately give any non-trivial approximation for our setting.

The only previous work that gives some guarantee for our setting is via \emph{non-clairvoyant} schedules. A non-clairvoyant schedule is one that schedules the jobs with no prior knowledge of their sizes at all (not even their distribution as in our model with stochastic jobs.) It is a folklore result that a non-clairvoyant schedule that $\alpha$-approximates the optimal clairvoyant schedule (one that knows all job sizes) immediately implies an adaptive policy that $\alpha$-approximates the optimal adaptive policy. Thus, in our setting, there exists a $2$-approximation for identical machines \cite{DBLP:journals/siamam/Graham69} and a $O(\log m)$-approximation for restricted assignment \cite{DBLP:journals/jal/AzarNR95} (all machines are identical, but each job can be assigned only to certain machines.) Note that trivial examples rule out any non-clairvoyant algorithm for unrelated machines with bounded approximation ratio (consider jobs with arbitrarily large size on some machines and size zero on all others.)\rud{add $\Omega(\sqrt{m})$ lower bound for non-clairvoyant related?} \rud{also can probably easily show matching upper bound}

\add{some previous work on routing}

\subsection{Our Results}

We go beyond non-clairvoyance and show that knowledge of job-size distributions allows us to improve on folklore results and overcome non-clairvoyant lower bounds. We give both offline- and online algorithms. In most cases, our algorithms are asymptotically tight with respect to the adaptivity gap or online lower bounds even for deterministic jobs. Our first result gives the first non-trivial approximation in the most general unrelated machines setting for load balancing. \add{diviation from classical optimal adaptive solution: We actually compare ourselves against an optimal solution that gains access to the processing time realizations upon placing a job on a machine.} 

\begin{theorem}\label{thm_unrel_lb_off}
	There exists an efficient offline algorithm that computes a non-adpative policy for load balancing on unrelated machines with stochastic jobs that $O(\frac{\log m}{\log \log m})$-approximates the optimal adaptive policy.
\end{theorem}

\begin{theorem}\label{thm_unrel_lb_on}
	There exists an efficient online algorithm that computes a non-adpative policy for load balancing on unrelated machines with stochastic jobs that $O(\log m)$-approximates the optimal adaptive policy.
\end{theorem}

Recall that there is a $\Omega(\frac{\log m}{\log \log m})$ lower bound on the adaptivity gap even for identical machines \cite{DBLP:journals/mor/Gupta0NS21}. Thus, \Cref{thm_unrel_lb_off} gives an asymptotically tight upper bound on the adaptivity gap between the optimal non-adaptive policy and the optimal adaptive policy. Similarly, there is a $\Omega(\log m)$ lower bound on the competitive ratio for online load balancing on unrelated machines even for deterministic jobs \cite{DBLP:journals/jal/AzarNR95}, so \Cref{thm_unrel_lb_on} is asymptotically optimal.

To improve on the above result, we need to use adaptivity. In the special case of related machines, we give a $O(1)$-approximation offline and a $O(\log \log m)$-approximation online.

\begin{theorem}\label{thm_rel_lb_off}
	There exists an efficient offline algorithm that computes an adaptive policy for load balancing on related machines with stochastic jobs that $O(1)$-approximates the optimal  adaptive policy.
\end{theorem}

\begin{theorem}\label{thm_rel_lb_on}
	There exists an efficient online algorithm that computes an adaptive policy for load balancing on related machines with stochastic jobs that $O(\log \log m)$-approximates the optimal adaptive policy.
\end{theorem}

For routing, we give non-adaptive policies that are $O(\frac{\log m}{\log \log m})$- and $O(\log m)$-approximate for the offline- and online settings, respectively.

\begin{theorem}\label{thm_route_off}\rud{we didn't prove this, but it should be straightforward (or we can leave it existential/inefficient}
    There exists an efficient offline algorithm that computes a non-adaptive policy for routing with stochastic jobs that $O(\frac{\log m}{\log \log m})$-approximates the optimal adaptive policy.
\end{theorem}

\begin{theorem}\label{thm_route_on}
    There exists an efficient online algorithm that computes a non-adaptive policy for routing with stochastic jobs that $O(\log m)$-approximates the optimal adaptive policy.
\end{theorem}

Both of these results are asymptotically tight. The former gives a tight upper bound on the adaptivity gap of \alert{...}\rud{should be straightforward to show $\Omega(\log m / \log \log m)$ gap as in identical machines} and is asymptotically optimal assuming \alert{...}  \addref. For the latter, there is a lower bound of $\Omega(\log m)$ on the competitive ratio of any algorithm even for deterministic jobs \cite{DBLP:journals/jal/AzarNR95}.

\subsection{Technical Overview}

\add{content}


\subsection{Related Work}

\add{other stochastic problems}

==> old/old_rel_off.tex <==
\section{Offline Load Balancing on Related Machines}\label{sec_off_rel} 

\fra{Started with this section because I need the lemma statement for related online machines.} 

\add{algorithm for smoothing the set of machines}

In this section, we improve on \Cref{thm_unrel_lb_off} in the special case of related machines, where each machine $i$ has a speed parameter $s_i > 0$ and each job $j$ an independent size $X_j$ such that $X_{ij} = \frac{X_j}{s_i}$. Recall that we gave a non-adaptive $O(\frac{\log m}{\log \log m})$-approximation for unrelated machines. However, the adaptivity gap is $\Omega(\frac{\log m}{\log \log m})$ even for identical machines (every machine has the same speed.) Thus, to improve on \Cref{thm_unrel_lb_off}, we need to use adaptivity.

The starting point of our improved algorithm is the same non-adaptive assignment generated by rounding $\lpgap$. We will not follow the non-adaptive assignment exactly; instead, if the non-adaptive assignment specifies $j \rightarrow i$, we adaptively assign $j$ to the least loaded machine with similar speed to $i$.

To formalize this idea, we define a notion of \emph{smoothed machines}. We show that by losing a constant factor in the approximation ratio, we may assume the machines are partitioned into at most $O(\log m)$ groups such that machines within a group have the same speed and the size of the groups shrinks geometrically. \rud{cite Im, Panigrahi and relate ours to theirs?}\fra{Probably. There will be a reviewer asking about the differences ...} Thus, by ``machines with similar speed to $i$,'' we mean machines in the same group.

\begin{comment}
Recall that we relax the optimal algorithms we compare our solutions to in the sense that they gain access to a job's realization by assigning the job to a machine. In particular, any such adaptive algorithm might base its decisions on this additional information. 
\end{comment}

\fra{I'd like to move the algorithm's description and its summary out of the proof of the lemma if you don't mind. Right now, you are mixing argumentation and algorithm in the proof, which is something one can avoid to make the argumentation cleaner.}

\begin{lem}[Machine Smoothing]\label{lem_rel_smooth}
    Let ~$\mathcal I$ be an instance of load balancing on $m$ related machines with stochastic jobs. By decreasing machine speeds and deleting machines, we can efficiently compute an instance  $\mathcal I_s$ of so-called ``smoothed machines'' and the same set of jobs with the following properties: 
    \begin{enumerate}[label=(\roman*)]
        \item The machines are partitioned into $m' = O(\log m)$ groups such that group $k$ consists of $m_k$ machines with speed exactly $s_k$ such that $s_1 < s_2 < \dots < s_{m'}$.\label{smoothed_prop_speeds}
        \item For all groups $1 \leq k < m'$, we have $m_k \geq \frac{3}{2} m_{k+1}$. \label{smoothed_prop_groups}
        \item $\Opt (\mathcal I_s) = O( \Opt (\mathcal I))$.\label{smoothed_prop_cost}
    \end{enumerate}
\end{lem}
\begin{proof}
    Consider the following algorithm to compute $\mathcal{I}_s$:
    
    \medskip
    \hrule
    \smallskip
    \hrule
    \smallskip
        	\begin{OneLiners}
        		\item[i.] We may assume by re-scaling that the fastest machine in $\mathcal{I}$ has speed exactly $1$. Delete all machines with speed less than $\frac{1}{m}$, so all machine speeds are in $[\frac{1}{m},1]$.
        		\item[ii.] Round the speeds of all remaining machines down to the nearest inverse power of $2$. Then partition the remaining machines into groups consisting of all those with the same speed. There are $O(\log m)$ distinct speeds and thus groups.
        		\item[iii.] Index the groups in increasing order of speed and consider them in this order. When considering group $k$, if $m_k < \frac{3}{2} m_{k+1}$, then delete group $k$, and move on to group $k+1$.
        		\item[iv.] Let $\mathcal{I}_s$ be the resulting machines along with the same jobs as the input instance $\mathcal{I}$.
            \end{OneLiners}
    \medskip
    \hrule
    \smallskip
    \hrule
    \medskip
    
    It is clear that the algorithm is efficient and outputs $\mathcal{I}_s$ satisfying \ref{smoothed_prop_speeds} and \ref{smoothed_prop_groups}. It remains to show \ref{smoothed_prop_cost}. To do so, we show that each step increases $\Opt$ by only a constant factor.
    
    Recall that $\Opt$ is an adaptive policy. On related machines, when an adaptive policy decides to schedule job $j$ on machine $i$, it immediately learns the realized value of $X_{ij}$, or equivalently $X_j = s_i \cdot X_{ij}$. It follows, we may assume the next scheduling decision of $\Opt$ is completely determined by the previously-realized $X_j$'s. In particular, if $\Opt$ decides to schedule $j$ on machine $i$, then we can modify $\Opt$ by scheduling $j$ on some other machine $i'$ and leaving the subsequent decisions (which in general depend on $X_j$) unchanged. Similarly, if we modify the speed of machine $i$, then this does not affect subsequent scheduling decisions.
    
    \begin{enumerate}
        \item[i.] Let $\Opt = \Opt(\mathcal{I})$ denote the initial optimal policy. Consider the following adaptive policy for the instance after step $i.$: If $\Opt$ schedules $j$ on $i$ such that $i$ is not deleted, then we also schedule $j$ on $i$. Otherwise, $\Opt$ schedules $j$ on $i$ such that $i$ is deleted for being too slow. Then we schedule $j$ on the fastest machine.
        
        For every realization of job sizes, the modified policy only increases the load of the fastest machine. We delete at most $m$ machines each having speed at most $\frac{1}{m}$. Thus, we schedule all jobs assigned to these machines on a machine that is at least $m$ times faster. The increase in load on the fastest machine is thus at most $m \cdot \frac{\Opt}{m} = \Opt$.
        \item[ii.] We decease the speed of each machine by at most a $2$-factor, so the makespan of the optimal policy increases by at most a $2$-factor. 
        \item[iii.] First, we note that we keep at least one group (the fastest one.) Consider any group $k$ that is deleted, and let $k' > k$ be the slowest subsequent group that is kept. Because we delete all groups between $k$ and $k'$, we have $m_k < (\frac{3}{2})^{k' - k} \cdot m_{k'}$. Further, because all groups have distinct speeds that differ by at least a $2$-factor, we also have $s_{k'} \geq 2^{k' - k} \cdot s_k$.
        
        Let $\Opt$ be the optimal policy after step ii. We re-assign the jobs that $\Opt$ schedules on group $k$ to group $k'$ as follows. Because $m_k < (\frac{3}{2})^{k' - k} \cdot m_{k'}$, we fix a mapping from the machines in group $k$ to those of $k'$ such that each machine in $k'$ is mapped to by at most $(\frac{3}{2})^{k' - k}$ machines in $k$. Then, when $\Opt$ schedules a job on a machine in group $k$, we instead schedule it on the machine it maps to in group $k'$. This completes the description of our modified policy.
        
        To bound the makespan, consider any machine $i$ in a kept group $k'$. We upper-bound the increase in load on $i$ due to re-assignments from slower deleted groups. For any deleted group $k < k'$, at most $(\frac{3}{2})^{k' - k}$ machines from group $k$ map to $i$. Each such machine in group $k$ under policy $\Opt$ has load at most $\Opt$. However, recall that $i$ is at least a $2^{k'-k}$-factor faster than any machine in group $k$, so the increase in load on machine $i$ due to deleted machines from group $k < k'$ is at most $(\frac{3}{2})^{k'-k} \cdot 2^{-(k' -k)} \cdot \Opt = (\frac{3}{4})^{k' -k} \cdot \Opt$. Summing over all $k < k'$, the total increase in load on a machine in group $k'$ is at most $\sum_{k < k'} (\frac{3}{4})^{k' -k} \cdot \Opt = O(\Opt)$.
    \end{enumerate}
\end{proof}

==> old/old_rel_on.tex <==
\section{Online Load Balancing On Related Machines}\label{sec_online_related}

% relies on machine smoothing 
% corollary from previous section? 

==> old/old_routing_on.tex <==
\section{Online Routing of Virtual Circuits}\label{sec_online_routing}

==> old/old_unrel_off.tex <==
\section{Warm Up: Offline load balancing on unrelated machines}\label{sec_unrel_off}

We illustrate the main ideas of our approach using the load balancing problem on unrelated machines. The goal of this section is to construct a non-adpative policy to prove \Cref{thm_unrel_lb_off}. We let $\Opt$ denote the optimal adaptive policy and its makespan.

First, we observe that if all job sizes were bounded with respect to $\mathbb{E}[\Opt]$ on every machine, then assigning jobs to machines such that each machine has expected load $O(\mathbb{E}[\Opt])$ gives the desired $O(\frac{\log m}{\log \log m})$-approximation. This is formalized in the next lemma.

\begin{lem}\label{lem_max_bound}\rud{I changed the lemma statement to a weaker multiplicative bound; I'm actually not sure if you can get an additive log/log log}\fra{For our online result we need the additive bound. However, there we only have $\EE[S_i] \leq O(\log m)$ and aim for $\EE[\max S_i] \leq O(\log m)$. Using the last Chernoff-Hoeffding inequality is sufficient.}
    Let $S_1, \dots, S_m$ be sums of random variables, each consisting of independent random variables bounded in $[0,\tau]$ for some $\tau > 0$ such that $\mathbb{E} [S_i] \leq \tau$ for all $i$. Then $\mathbb{E} [\max_i S_i] = O(\tau \cdot \frac{\log m}{\log \log m})$.
\end{lem}
\begin{proof}
    By re-scaling, it suffices to prove the lemma for $\tau = 1$. Consider one such sum, say $S = \sum_j X_j$, where the $X_j$'s are independent and bounded in $[0, 1]$. We use Bennett's inequality (\Cref{prop_bennett}) to bound the upper-tail of $S$. Applying Bennett's inequality to $S - \mathbb{E}[S]$ with $a = 1$ and $\sigma^2 = \sum_j \mathbb{E}\big[(X_j - \mathbb{E}[X_j])^2\big] \leq \sum_j \mathbb{E}[X_j^2] \leq \sum_j \mathbb{E}[X_j] \leq 1$ gives for any $t \geq 0$:
    \[\mathbb{P}(S > 1 + t) \leq \mathbb{P}(S > \mathbb{E}[S]+t) \leq \exp\big(-(1 + t) \log (1  + t) + t\big)  = \frac{e^t}{(1 + t)^{1 + t}}.\]
    In particular, for $\ell = O(\frac{\log m}{\log \log m})$ large enough, we have for any $t \geq 0$:
    \begin{equation*}
        \mathbb{P}(S > 1 + \ell + t) \leq \frac{e^{\ell + t}}{(1 + \ell + t)^{1 + \ell + t}} \leq \frac{e^\ell}{\ell^\ell} \cdot \frac{e^t}{\ell^t} = O\big(\frac{1}{m}\big) \cdot e^{-t}.
    \end{equation*}
    This tail bound holds for all $S_1, \dots, S_m$. Union-bounding over all $m$ sums gives:
    \begin{align*}
        \mathbb{E} [\max_i S_i] &= \int_0^\infty \mathbb{P}( \max_i S_i > t) \cdot dt\\
        &\leq (1 + \ell) + \int_0^\infty \mathbb{P}( \max_i S_i > 1+ \ell + t) \cdot dt\\
        &\leq (1 + \ell) + \sum_i \int_0^\infty \mathbb{P}(S_i > 1 + \ell + t) \cdot dt\\
        &= (1 + \ell) + m \cdot O\big(\frac{1}{m}\big) \int_0^\infty e^{-t} \cdot dt = O(\ell) = O \big(\frac{\log m}{\log \log m} \big).
    \end{align*}
\end{proof}

However, what if each $X_{ij}$ is not bounded in $[0 ,\mathbb{E}[\Opt]]$? In general, we have no upper bound on $X_{ij}$, so we cannot apply \Cref{lem_max_bound} to the jobs directly. We turn these unbounded random variables into bounded ones in a standard way by splitting each job into \emph{truncated} and \emph{exceptional} parts.

\begin{definition}[Truncated and Exceptional Parts]\label{def_truncated_and_exceptional}
    Let $\tau \geq 0$ be a fixed threshold. For any job $X_{ij}$, its truncated part (with respect to threshold $\tau$) is $X_{ij}^T = X_{ij} \cdot \one_{X_{ij} < \tau}$. Similarly, its exceptional part is $X_{ij}^E = X_{ij} \cdot \one_{X_{ij} \geq \tau}$. Note that $X_{ij} = X_{ij}^T + X_{ij}^E$.
\end{definition}\fra{I introduced a command to make the indicator function blackboard as well. one $\rightarrow \one$}

It is immediate that the truncated parts $X_{ij}^T$ are bounded in $[0, \tau]$, so taking $\tau = O(\mathbb{E}[\Opt])$, we can apply \Cref{lem_max_bound} to control the contribution of truncated parts to the makespan. It remains to bound the contribution of exceptional parts. Concretely, let $\{j \rightarrow i\}$ be the event that some fixed policy assigns jobs $j$ to machine $i$. We want to control the quantity
\[\mathbb{E}\Big[\max_i \sum_{j \rightarrow i}  X_{ij}^E\Big].\]
Because we have no reasonable bound on the $X_{ij}^E$'s, for non-adaptive policies we can only trivially upper bound the expected max by the sum \rud{I think this upper bound is tight up to constants; not sure if worth giving example}
\[\mathbb{E}\Big[\max_i \sum_{j \rightarrow i}  X_{ij}^E\Big] \leq \sum_i \sum_{j \rightarrow i}  \mathbb{E} \big[X_{ij}^E\big].\]
We call this final expression the \emph{total (expected) exceptional load}. Thus, to obtain our final non-adaptive policy, our goal is to assign jobs to machines such that the expected truncated load on each machine and the total expected exceptional load are both at most $O(\mathbb{E}[\Opt])$. This subproblem is exactly an instance of the generalized assignment (GAP) problem, which has the following natural LP relaxation. The variable $y_{ij}$ denotes assigning job $j$ to machine $i$. We take our threshold between the truncated- and exceptional parts to be $\tau$ and $C$ some parameter. 

    \begin{equation}\tag{$\lpgap$}\label{eq_lpgap}
       \begin{array}{rll}
         \sum_{ij} \mathbb{E} [X_{ij}^E] \cdot y_{ij} & \leq C \\
         \sum_j \mathbb{E} [X_{ij}^T] \cdot y_{ij} & \leq \tau &\quad\forall i\\
         \sum_i y_{ij} &  = 1 &\quad\forall j\\
         y_{ij} & \geq 0 &\quad\forall i,j
        \end{array} 
    \end{equation}
    
We comment that the standard GAP LP also includes pruning constraints of the form $y_{ij} = 0$ for $i,j$ such that $\mathbb{E} [X_{ij}^T] > \tau$, but by definition of truncated parts, we have $\mathbb{E} [X_{ij}^T] < \tau$. Thus, the pruning constraints are unnecessary.

It is known that $\eqref{eq_lpgap}$ \fra{Using eqref\{eq\_lpgap\} you can now refer to the lp} can be efficiently rounded with small additive violation in the second constraint \cite{DBLP:journals/mp/ShmoysT93}. Thus, if $\lpgap$ is feasible, then we can obtain an integral solution (i.e. a non-adaptive policy) whose expected truncated load is $O(\tau)$ per machine and total expected exceptional load is at most $C$. Using our above bounds on the truncated- and exceptional parts, the expected makespan of this policy is $O(\tau \frac{\log m}{\log \log m} + C)$.

To obtain the desired $O(\frac{\log m}{\log \log m})$-approximation, we need to take $\tau = O(\mathbb{E}[\Opt])$. How small can we take $C$ for $\lpgap$ to be feasible? If we were instead approximating the optimal \emph{non-adaptive} policy, then we could take $C = O(\mathbb{E}[\Opt])$ using known lower bounds on the optimal non-adaptive policy \cite{DBLP:journals/siamcomp/KleinbergRT00, DBLP:journals/mor/Gupta0NS21}. However, the next example shows that the optimal adaptive policy can have total expected exceptional load $\Omega(m \cdot \mathbb{E} [\Opt])$.

\begin{example}\label{ex_except_lower}
    We define an instance on \emph{related} machines. Recall that for related machines, each machine $i$ has a speed $s_i$ and each job $j$ has processing time $X_j$ such that $X_{ij} = \frac{X_j}{s_i}$.
        
    Our instance has one ``fast'' machine with speed $1$ and $m-1$ ``slow'' machines each with speed $\frac{1}{\tau m}$, where $\tau > 0$ is the truncation threshold. There are $m$ jobs. One is stochastic with processing time $\tau \cdot Ber(\frac{1}{\tau})$ and the remaining $m-1$ jobs are deterministic with processing time $\frac{1}{m}$.
        
    The optimal adaptive policy is to first schedule the stochastic job on the fast machine. If its realized size is $0$, then we schedule all deterministic jobs on the fast machine. Otherwise its realized size is $\tau$. In this case, we schedule one deterministic job on each slow machine. This gives $\mathbb{E}[\Opt] = (1 - \frac{1}{\tau})(\frac{m-1}{m}) + \frac{1}{\tau} \cdot \tau = \Theta(1)$. However, the total expected exceptional load (with respect to threshold $\tau$) is $\sum_{i,j} \mathbb{E} [X_{ij}^E \cdot \one_{j \rightarrow i}] = \frac{1}{\tau}(m \tau) = m$.
\end{example}

The issue in \Cref{ex_except_lower} is that the exceptional parts are scheduled in a correlated way such that they do not greatly effect the expected makespan. We solve this issue by showing that there is a near-optimal adaptive policy that has small total expected exceptional load. Although in the example we can achieve this by simply scheduling all jobs on the fast machine, this does not generalize to unrelated machines. On unrelated machines, we modify the optimal policy by ``restarting'' whenever an exceptional job is encountered. This is one of the main technical innovations of our work, and it is given in the next theorem.
    
\begin{theorem}\label{thm_adap_restart}
    For load balancing on unrelated machines with stochastic jobs, there exists an adaptive policy with expected makespan and total expected exceptional load at most $2 \cdot \mathbb{E} [\Opt]$ with respect to any truncation threshold $\tau \geq 2 \cdot \mathbb{E}[\Opt]$. 
\end{theorem}\fra{I believe that this theorem also holds for the generalization to load balancing (altough here, we only consider the contribution of $\max_i X_{ij}^E(c)$ for some configuration $c$ to the exceptional load. Do we want to state and prove the theorem in its full generality or do we add another theorem on load balancing down the road (potentially without proving it)?}

\begin{proof}
    We prove the theorem by induction on the number of jobs $n = 0,1, \dots$. The base case $n = 0$ is trivial. For $n > 0$, let $J$ denote the set of jobs. For any subset $J' \subset J$, we let $\Opt(J')$ denote the optimal adaptive policy (and its makespan) on the set of jobs $J'$. Consider a fixed truncation threshold $\tau \geq 2 \mathbb{E} [\Opt(J)]$. We construct the desired adaptive policy as follows:
    
    \medskip
    \hrule
    \smallskip
    \hrule
    \smallskip
        	\begin{OneLiners}
        		\item[i.] Run policy $\Opt(J)$.
        		\item[ii.] At the first decision that schedules an exceptional job (one that has realized size at least $\tau$,) we stop running $\Opt(J)$. Note that if no decision schedules an exceptional job, then we run $\Opt(J)$ to completion, and we are done.
        		\item[iii.] Let $R \subset J$ denote the remaining set of unscheduled jobs. We have $\lvert R \rvert < \lvert J \rvert$, so let $S(R)$ denote the policy on $R$ guaranteed by \Cref{thm_adap_restart} by induction. Then run policy $S(R)$ to completion.
            \end{OneLiners}
    \medskip
    \hrule
    \smallskip
    \hrule
    \medskip

    The makespan of this policy is at most $\Opt(J) + S(R)$, where we follow the convention that $R = \emptyset$ if no decision schedules an exceptional job when running $\Opt(J)$. In expectation, we have:
        \begin{align*}
            \mathbb{E} [S(R)] &= \sum_{J' \subset J} \mathbb{E}[S(R) \mid R = J'] \cdot \mathbb{P}(R = J')\\
            &= \sum_{J' \subset J} \mathbb{E} [S(J')] \cdot \mathbb{P}(R = J')\\
            & \leq 2 \sum_{J' \subset J} \mathbb{E} [\Opt(J')] \cdot \mathbb{P}(R = J')\\
            & \leq 2 \cdot \mathbb{E} [\Opt(J)] \cdot \mathbb{P}(R \neq \emptyset).
        \end{align*}
    In the second line, we use the fact that the realizations of the remaining jobs in $J'$ are independent of the event $R = J'$. The third line uses the inductive hypothesis. The final line uses $J' \subset J$, so $\mathbb{E} [\Opt(J')] \leq \mathbb{E} [\Opt(J)]$, and $\Opt(\emptyset) = 0$. Note that on the event $R \neq \emptyset$, we have that $\Opt(J)$ schedules a job that becomes exceptional, so $\Opt(J) \geq \tau \cdot \one_{R \neq \emptyset} \geq 2 \cdot \mathbb{E} [\Opt(J)] \cdot \one_{R \neq \emptyset}$. Taking expectations gives $\mathbb{P}(R \neq \emptyset) \leq \frac{1}{2}$. To conclude, we can upper bound the expected makespan of our policy by:
        \[\mathbb{E} [\Opt(J)] + \mathbb{E} [S(R)] \leq \mathbb{E} [\Opt(J)] + 2 \cdot \mathbb{E} [\Opt(J)] \cdot \mathbb{P}(R \neq \emptyset) \leq 2 \mathbb{E} [\Opt(J)].\]
        
    The computation for the total expected exceptional load is similar. We let $j \rightarrow i$ denote the event that our policy schedules job $j$ on machine $i$. Then we can split the exceptional load into two parts based on if a job is scheduled by $\Opt(J)$ or $S(R)$:
    \[\sum_{i,j} X_{ij}^E \cdot \one_{j \rightarrow i} = \sum_{i,j} X_{ij}^E \cdot \one_{j \xrightarrow{J} i} + \sum_{i,j} X_{ij}^E \cdot \one_{j \xrightarrow{R} i},\]
    where we let $j \xrightarrow{J} i$ and $j \xrightarrow{R} i$ denote the events that $j$ is scheduled on machine $i$ by $\Opt(J)$ up to and including the first exceptional job, or by $S(R)$ after the first exceptional job, respectively.
        
    We first bound the former term, corresponding to the jobs scheduling up to and including the first exceptional job in $\Opt(J)$. On the event that no exceptional job is scheduled, we have $\sum_{i,j} X_{ij}^E \cdot \one_{j \xrightarrow{J} i} = 0$ by definition. Otherwise, let $j^* \rightarrow i^*$ be the first (and only) exceptional job scheduled by $\Opt(J)$. Then $\sum_{i,j} X_{ij}^E \cdot \one_{j \xrightarrow{J} i} = X_{i^* j^*}^E \leq \Opt(J)$. Combining these two bounds gives $\mathbb{E} [\sum_{i,j} X_{ij}^E \cdot \one_{j \xrightarrow{J} i}] \leq \mathbb{E} [\Opt(J)]$.
        
    For the latter term, we again condition on the events $R = J'$ and apply the inductive hypothesis. We note that all exceptional jobs are with respect to the fixed $\tau \geq 2 \cdot \mathbb{E} [\Opt(J)] \geq 2 \cdot \mathbb{E} [\Opt(J')]$ for $J' \subset J$.
        \begin{align*}
            \mathbb{E} \Big[\sum_{i,j} X_{ij}^E \cdot \one_{j \xrightarrow{R} i}\Big] &= \sum_{J' \subset J} \mathbb{E} \Big[\sum_{i,j} X_{ij}^E \cdot \one_{j \xrightarrow{R} i} \mid R = J'\Big] \cdot \mathbb{P}(R = J')\\
            &= \sum_{J' \subset J} \mathbb{E}\Big[ \sum_{i,j \in J'} X_{ij}^E \cdot \one_{j \xrightarrow{J'} i}\Big] \cdot \mathbb{P}(R = J')\\
            &\leq 2 \sum_{J' \subset J} \mathbb{E} [\Opt(J')] \cdot \mathbb{P}(R = J')\\
            &\leq 2 \mathbb{E} [\Opt(J)] \cdot \mathbb{P}(R \neq \emptyset) \leq \mathbb{E} [\Opt(J)].
        \end{align*}
        Note that we define $j \xrightarrow{J'} i$ to be the event that the policy $S(J')$ schedules $j$ on $i$. In conclusion, by combining our bounds for these two terms we have:
        \[\sum_{i,j} \mathbb{E} \big[X_{ij}^E \cdot \one_{j \rightarrow i}\big] = \sum_{i,j} \mathbb{E} \big[X_{ij}^E \cdot \one_{j \xrightarrow{J} i}\big] + \sum_{i,j} \mathbb{E} \big[X_{ij}^E \cdot \one_{j \xrightarrow{R} i}\big] \leq \mathbb{E} [\Opt(J)] + \mathbb{E} [\Opt(J)].\]
\end{proof}

Using this near-optimal policy, we can show $\lpgap$ is feasible for small $C$ by losing only a constant factor in the makespan/threshold.

\begin{lem}\label{lem_gaplp_feasible}
    $\lpgap$ is feasible for any $\tau, C \geq 2 \cdot \mathbb{E}[\Opt]$.
\end{lem}
\begin{proof}
    Consider the adaptive policy guaranteed by \Cref{thm_adap_restart}, and let the events $j \rightarrow i$ be with respect to this policy. We consider the natural setting of the $y$-variables given this policy: for all $i,j$, we take $y_{ij} = \mathbb{P}(j \rightarrow i)$. It is clear that $\sum_i y_{ij} = 1$ for all $j$ and $0 \leq y_{ij} \leq 1$ for all $i,j$. It remains to verify the exceptional- and truncated load constraints. For the exceptional constraint:
    \[\sum_{ij} \mathbb{E}[X_{ij}^E] \cdot y_{ij} = \sum_{ij} \mathbb{E}[X_{ij}^E \cdot \one_{j \rightarrow i}] \leq 2 \cdot \mathbb{E}[\Opt] \leq C,\]
    where in the first step we use the fact that the decision to schedule job $j$ on machine $i$ is independent of its realization, and in the second we use the properties of the policy. Similarly, for the truncated constraint for each $i$:
    \[\sum_{j} \mathbb{E}[X_{ij}^T] \cdot y_{ij} = \sum_{j} \mathbb{E}[X_{ij}^T \cdot \one_{j \rightarrow i}] \leq 2 \cdot \mathbb{E}[\Opt] \leq \tau.\]
\end{proof}




\add{final alg; not sure best way to present guess-and-double.}


\begin{lem}\label{lem_guess_and_double}
    \add{lemma statement; proof probably in appendix.}
\end{lem}
\fra{needed something to refer to}


\begin{comment}
Using this near-optimal policy, we can give a feasible solution to $\lpunrel$.
    
    \begin{cor}\label{cor_lpunrel_feasible}
        $\lpunrel$ is feasible for $\tau, C \geq 2 \mathbb{E} Opt$.
    \end{cor}
    \begin{proof}
        Let $S$ be the instant adaptive policy guaranteed by \Cref{thm_adap_restart}. Consider the setting of the $y$-variables such that $y_{ij} = \mathbb{P}(j \rightarrow i)$, where the event $j \rightarrow i$ is with respect to policy $S$. We show that this setting is feasible for $\lpunrel$ with $\tau, C \geq 2 \mathbb{E} Opt$. First it is immediate that $0 \leq y_{ij} \leq 1$ for all $i,j$ and $\sum_i y_{ij} = 1$ for all $j$, because $S$ schedules each job with probability one.
        
        For the exceptional job constraint:
        \[\sum_{ij} \mathbb{E} X_{ij}^E y_{ij} = \sum_{ij} \mathbb{E} X_{ij}^E \one_{j \rightarrow i} \leq 2\mathbb{E} Opt,\]
        where we use the fact that $j \rightarrow i$ is independent from the realization of $X_{ij}$ and the properties of $S$ guaranteed by \Cref{thm_adap_restart}. Similarly, for the truncated job constraint:
        \[\sum_j \mathbb{E} X_{ij}^T y_{ij} \leq \sum_j \mathbb{E} X_{ij} \one_{j \rightarrow i} \leq 2 \mathbb{E} Opt,\] where the second inequality follows because the expected makespan of $S$ is at most $2 \mathbb{E} Opt$ by \Cref{thm_adap_restart} and $\sum_j \mathbb{E} X_{ij} \one_{j \rightarrow i}$ is exactly the expected load of machine $i$.
    \end{proof}
    
    \subsection{Algorithm and Proof of \Cref{thm_unrel_lb_off}}
    
    Now we are ready to combine our GAP LP (\Cref{lem_lpunrel_bound}), structural characterization of near-optimal policies (\Cref{cor_lpunrel_feasible}), and guess-and-double framework to state our complete algorithm. This will be the algorithm guaranteed by \Cref{thm_unrel_lb_off}
    
    By using guess-and-double, it suffices to give an efficient algorithm that either:
    \begin{itemize}
        \item outputs a non-adaptive policy with expected makespan $O(\log m)$, or
        \item certifies that $\mathbb{E} Opt = \Omega(1)$.
    \end{itemize}
    For this subproblem, our algorithm is the following:
    \begin{enumerate}
        \item Try to solve $\lpunrel$ with $\tau, C = 2$.
        \item If $\lpunrel$ is feasible, then run the algorithm guaranteed by \Cref{lem_lpunrel_bound}, and output the resulting non-adaptive policy with expected makespan $O(\log m)$.
        \item Otherwise, $\lpunrel$ is infeasible, so \Cref{cor_lpunrel_feasible} implies $\mathbb{E} Opt > 1$.
    \end{enumerate}
    It is clear that the above algorithm is efficient and solves the subproblem. This completes the proof of \Cref{thm_unrel_lb_off}.
\end{comment}

==> old/old_unrel_on.tex <==
\section{Online Load Balancing On Unrelated Machines}\label{sec_online_unrelated}

\fra{Work in progress, do not read.} 

Building on the blocks we developed in the previous section, we now address \emph{online} load balancing on unrelated machines. The goal of this section is to prove \Cref{thm_unrel_ub_on}. 

Assume for now that we have an accurate guess of the final $\EE[\Opt]$, denoted by~$\lambda^*$. We will later drop this assumption by employing a standard guess-and-double framework. Given~$\lambda^*$, we know by \Cref{thm_adap_restart} that $\lpgap$ admits a feasible solution for the choices~$C = \tau = 2\lambda^*$. More precisely, we use that there is an assignment $(y_{ij})_{ij}$ of jobs to machines satisfying 
\begin{align*}
    \sum_{i, j} \EE[X_{ij}^E] \cdot y_{ij} & \leq 2 \lambda^* \\
    \sum_{j} \EE[x_{ij}^T] \cdot y_{ij} & \leq 2 \lambda^* \qquad \forall i. 
\end{align*}
Let us denote this near-optimal assignment by~$\Opt'$. Using a potential function, we find an integral assignment online that violates these two constraints by a factor at most~$O(\log m)$, hence proving the desired result. 

Employing a potential function for online load balancing is a common idea and was first used by \cite{DBLP:journals/jal/AzarNR95} for online load balancing when the request sizes become known to the scheduler upon arrival of a request. In order to generalize this idea to stochastic jobs, or requests, we transform our jobs into~$(m+1)$-dimensional load vectors that simultaneously represent the contribution of a job-to-machine assignment to the truncated load on that machine as well as the total exception load incurred by all machines. To this end, upon arrival of job~$j$, we create the following~$m$ load vectors: 
\begin{equation*}
    v_{ij}(i') = 
    \begin{cases}\EE \big [X_{i'j} \cdot \one_{X_{i'j} \geq 2 \lambda^*}\big] = \EE \big [X_{i'j}^E \big] & \textup{ if } i = 0 \\ 
        \EE \big [X_{i'j} \cdot \one_{X_{i'j} < 2 \lambda^*}\big] = \EE \big [X_{i'j}^T \big] & \textup{ if } i = i' \\ 
        0 & \textup{ otherwise.}
    \end{cases}
\end{equation*} 
Here, dimension~$0$ represents the total exceptional load. 

Similarly, let~$\load_{ij}$ denote the expected load on machine~$i$, $0 \leq i \leq m$ after job~$j$ has been assigned. Let~$\phi(\load) = \sum_{i=0}^m (3/2)^{\load_i / (2\lambda^*)}$ be the potential of some load vector~$\load$. Upon arrival of job~$j+1$, assign~$j+1$ to machine~$i'$, where~$i'$ minimizes~$\phi(\load_j + v(i')) - \phi(\load_j)$ and define~$\load_{j+1}$ accordingly. 

Assuming a correct guess~$\lambda^*$ for~$\EE[\Opt]$, we show the following lemma. 

\begin{lem}\label{lem_unrel_on_potential} 
    If~$\EE[\Opt] \leq \lambda^*$, then the online assignment~$\mathcal{A}$ satisfies~$\EE[\mathcal A] \leq O(\log m) \lambda^*$.  
\end{lem} 

Note that there is a lower bound of~$O(\log m)$ for any deterministic online algorithm for load balancing on unrelated machines, even when the processing times are deterministic, implying that the competitive ratio is best possible up to multiplicative constants. 

Combining the algorithm with a standard doubling technique proves \Cref{thm_unrel_ub_on}. We summarize the algorithm in \Cref{alg_on_unrel}. \fra{Remove guess and double, will appear in appendix}
\begin{algorithm}
    \DontPrintSemicolon
    \caption{Online Load Balancing on Unrelated Machines}
    \label{alg_on_unrel}  
    $\load \leftarrow 0$, $\lambda \leftarrow 1$, $h \leftarrow 0$ \;
    \textbf{upon arrival of job $\mathbf j$:} \;
    $v_j(i) \leftarrow$ load vector for $j$ on machine $i$ \;
    $i^* \leftarrow \arg \min_i \{ \phi(\load + v(i)) - \phi(\load)$ \}\;
    \uIf{
    $\load_{i^*} + v_{i^*j}(i^*) \leq O(\log m) \lambda$ {\normalfont \bfseries and} $\load_0 + v_{0j}(i^*) \leq O(\log m) \lambda$}{
    assign $j$ to $i^*$ \;
    $\load \leftarrow \load + v_j(i^*)$ \;    }
    \Else{
    $\load \leftarrow 0$, $\lambda \leftarrow 2 \lambda$, $h \leftarrow h + 1$ \;
    go to Line 2 \;
    }
\end{algorithm}

\begin{proof}
    Let~$v_j$ denote the load vector corresponding to the assignment of job~$j$ by~$\mathcal A$. Recall that the load incurred by these vectors on machine~$0$ captures the total exceptional load of the algorithm's assignment while their load on machine~$i$ reflects the truncated load on~$i$. First, we show that~$\sum_{j=1}^n v_{ij} \leq O(\log m) \lambda^*$ holds for each machine~$0 \leq i \leq  m$ before using this fact to prove the theorem. 
    
    Let~$\Opt'$ denote again the near-optimal assignment, and let~$v_j^*$ be the load vector corresponding to~$j$'s assignment by~$\Opt'$. Note that \Cref{thm_adap_restart} guarantees~$\sum_{j=1}^n v_{ij} ^* \leq 2 \lambda^*$ for every machine~$0 \leq i \leq m$.    
    
    By letting~$\load_0 = 0$ be the all-zero vector, we have~$\phi(\load_0) = m+1$. This allows us to bound the increase in the potential function as follows 
    \begin{align*}
        \phi(\load_n) - \phi(\load_0) & = \sum_{j=1}^n \sum_{i=0}^m \frac32^{\load_{ij}/(2\lambda^*)} \Big( \frac32^{v_{ij}/(2\lambda^*)} -1 \Big) \\ 
        & \leq \sum_{j=1}^n \sum_{i=0}^m  \frac32^{\load_{ij}/(2\lambda^*)} \Big( \frac32^{v_{ij}^*/(2\lambda^*)} -1 \Big) \\ 
       &  \leq \sum_{i=0}^m \frac32^{\load_{in}/(2\lambda^*)} \sum_{j=1}^n \Big( \frac32^{v_{ij}^*/(2\lambda^*)} -1 \Big), 
       \intertext{where the first inequality holds because the algorithm's assignment minimizes the increase in potential and the second inequality holds because the load on machine~$i$ only increases over time. By a simple algebraic computation, we can bound 
       $ \frac32^{(v_{ij}^*/(2\lambda^*)} -1 \leq \frac12 \frac{v_{ij}^*}{2\lambda^*}$. As the load vectors~$v_j^*$ correspond to the near-optimal solution~$\Opt'$, we know that~$\sum_j \frac{v_{ij}^*}{2\lambda^*} \leq 1$. Hence,}
       \phi(\load_n) - \phi(\load_0) & \leq \frac12 \sum_{i=0}^m \frac32^{\load_{in}/(2\lambda^*)} = \frac12 \phi(\load_n). 
   \end{align*}
    After rearranging, we get $\phi(\load_n) \leq 2 \phi(\load_0) = 2(m+1)$. Inserting the definition of the load vectors~$v_j$, we get 
    \begin{equation*}
        \sum_{i=1}^m 
        \frac{3}{2}^{\sum_{j \stackrel{\mathcal A}{\longrightarrow} i} \EE[X_{ij}^T]/ (2\lambda^*)} + \frac{3}{2}^{\sum_{i=1}^m \sum_{j \stackrel{\mathcal A}{\longrightarrow} i} \EE[X_{ij}^E]/(2\lambda^*)} \leq 2(m+1) 
    \end{equation*}
    Taking logarithms, this already implies the desired bound on the total exceptional load: 
    \begin{equation}\label{eq_unrel_on_excep}
        \EE\Bigg[ \max_{1 \leq i \leq m} \sum_{j \stackrel{\mathcal A}{\longrightarrow} i} X_{ij}^E\Bigg] \leq \sum_{i=1}^m \sum_{j \stackrel{\mathcal A}{\longrightarrow} i} \EE[X_{ij}^E] \leq O(\log m) \lambda^*.
    \end{equation}
    Similarly, for the truncated load~$\load_i^T$ on machine~$i$, we obtain 
    \[
        \EE[\load_i^T] = \sum_{j \stackrel{\mathcal A}{\longrightarrow} i} \EE[X_{ij}^T] \leq \log_{3/2}(2m + 2) \lambda^*.
    \]
    Using \Cref{lem_chernoff} for~$t > 4 e \log_{3/2}(2m + 2) \lambda^*$, we have~$\PP[\load_i^T > t] < 2^t$ because the variables~$X_{ij}^T$ are independent and bounded in~$[0,2\lambda^*]$. \rud{we can probably replace this computation with \Cref{lem_max_bound}. Just kidding, now the lemma is too weak so your idea is needed}\fra{Let me think about this.} Therefore, \begin{align*}
        \EE\Big[ \max_{1 \leq i \leq m} \load_i^T \Big] \notag
        & = \int_{0}^\infty \PP\Big[ \max_{1 \leq i \leq m} \load_i^T  > t  \Big] dt \\
        & \leq O(\log m)\lambda^* + \int_{O(\log m) }^\infty  \PP\Big[ \max_{1 \leq i \leq m} \load_i^T  > t  \Big] dt \\
        & \leq O(\log m)\lambda^* + \sum_{i=1}^m \int_{O(\log m)}^\infty \PP\Big[ \load_i^T  > t  \Big] dt \\
        & \leq O(\log m)\lambda^* + m \int_{O(\log m)}^\infty 2^t dt \\
        & = O(\log m)\lambda^*. 
    \end{align*}
    Combining this with Equation~\eqref{eq_unrel_on_excep} concludes the proof.
\end{proof}











==> old/split_config_on.tex <==


\subsection{Online Deterministic Requests}

It is natural to consider \emph{online configuration balancing} where the~$n$ requests arrive online one by one, and for each request, one configuration has to be irrevocably selected before the next request appears. In the following, we present an online algorithm for configuration balancing that achieves a competitive ratio of~$O(\log m)$, which is best possible due to the lower bound of~$\Omega(\log m)$ on the competitive ratio of any deterministic algorithm for online load balancing on unrelated machines \cite{DBLP:journals/jal/AzarNR95}. 

To highlight our algorithmic ideas, we focus on deterministic requests in this section before we show how to generalize our results to stochastic requests in the next section. The first ingredient is the observation that we can employ a classical doubling scheme and assume that we have a good guess~$\lambda$ on the optimal solution~$\Opt$. Formally, we will design an online algorithm with parameter~$\lambda$ such that the load on no resource exceeds~$\alpha \lambda$, unless~$\lambda < \Opt$. 

\begin{lem}\label{lem_guess_and_double}
    Suppose there is an online algorithm~$\Alg$ for online configuration balancing that never creates a maximum load greater than~$\alpha \lambda$ as long as~$\Opt \leq \lambda$. Then, there is a~$4 \alpha$-competitive algorithm for online configuration balancing.  
\end{lem}

The lemma can be proven analogously to its virtual-circuit-routing counterpart as described in \cite{AspnesAFPW97}. Hence, we omit the proof for conciseness. 


The key ingredient is to notice that the classical approach of using a potential function can be generalized to online configuration balancing. Based on minimizing the increase in the potential, the online algorithm is then able to greedily choose the load configuration for request~$j$. Aspnes et al.~\cite{AspnesAFPW97} are the first to employ this approach for online load balancing problems, more precisely for online virtual circuit routing. 

Let~$\load_{ij}$ denote the load on resource~$i \in [m]$ \emph{after} the online algorithm chose a configuration for request~$j$, where~$\load_{i0} := 0$.  Let~$\phi(\load) = \sum_{i=1}^m (3/2)^{\load_i / \lambda}$ be the potential of load vector~$\load$. 

The algorithm works as follows: Upon arrival of request~$j+1$, we would like to choose the configuration~$c_{j+1} \in [q_{j+1}]$ that minimizes~$\phi(\load_j + x_{j+1}(c)) - \phi(\load_j)$. If indeed~$\load_{ij} + x_{i j+1}(c_{j+1}) \leq O( \log m) \lambda$ holds for all resources~$i$, we assign configuration~$c_{j+1}$ to request~$j+1$ and update the load vector~$\load_{j+1} \leftarrow \load_j + x_{j+1}(c_{j+1})$. If~$\load_{ij} + x_{ij+1} > O(\log m) \lambda$ for some resource~$i$, we return~$\Opt > \lambda$. We summarize the algorithm below.

\begin{algorithm}
    \DontPrintSemicolon
    \caption{Online Configuration Balancing}
    \label{alg_on_config}  
    \textbf{upon arrival of request $j$}\;
    $c_j \leftarrow \arg \min_i \{ \phi(\load + x(c)) - \phi(\load)$\}\;
    \uIf{
    $\load_i + x_{ij}(c_j) \leq O(\log m) \lambda$ for all $i$}{
    choose $c_j$ for $j$ \;
    $\load \leftarrow \load + x_j(c_j)$ \;    }
    \Else{
    fail \;
    }
\end{algorithm}

For analyzing the competitive ratio of this algorithm, we compare its maximum load with the objective function value of the linear program~\eqref{eq_lpconfig}, the deterministic counterpart of~\eqref{eq_lpstochconfig}. The variables~$y_{cj}$ represent the fractional extend to which configuration~$c$ is chosen for request~$j\in[n]$, and the first constraint ensures that these fractions sum up to one. The second set of constraints bound the load on resource~$i \in [m]$. This LP clearly is a relaxation of offline configuration balancing, which can be encoded by adding integrality constraints on the~$y_{cj}$ variables to the LP.  
\begin{equation}\tag{$\lpdetconfig$}\label{eq_lpconfig}
   \begin{array}{rll}
     \sum_{c=1}^{q_j} y_{cj} &  = 1 &\quad\forall~j\in[n] \\
     \sum_{j=1}^n \sum_{c=1}^{q_j} x_{ij}(c) \cdot y_{cj}  &  \leq \lambda &\quad\forall~i\in[m] \\
     y_{cj} & = 0 & \quad \forall~ j \in [n], \forall~c \in [q_j]: \exists~i: x_{ij}(c) > \lambda \\ 
     y_{cj} & \geq 0 & \quad \forall~j\in[n], \forall~c \in [q_j] 
    \end{array} 
\end{equation}

We point out that this LP has an integrality gap of~$\Omega(\log m)$, which follows immediately from the path assignment LP for virtual circuit routing \addref. Hence, a straightforward analysis of \Cref{alg_on_config} using \eqref{eq_lpconfig} yields a competitive factor of~$O(\log^2 m)$, where one factor~$O(\log m)$ is due to the aforementioned integrality gap while the second factor~$O(\log m)$ is due to the use of the potential function. Crucially, the particular choices of \Cref{alg_on_config} allow us to directly compare the algorithm's solution to \emph{any} (not necessarily integral) feasible solution of~\eqref{eq_lpconfig}, implying a tight competitive ratio of~$O(\log m)$. 

\begin{theorem}\label{thm_dcb_on}
    If~\eqref{eq_lpconfig} is feasible for~$\lambda >0$, then \Cref{alg_on_config} guarantees a maximum load $O(\log m)\lambda$.  
\end{theorem}

\begin{proof}
    Let~$(y_{cj}) \in [0,1]$ be a feasible solution to~\eqref{eq_lpconfig}. Since \Cref{alg_on_config} chooses a configuration~$c_j$ minimizing the increase in potential, we have~$\phi(\load_{j-1} + x_j(c_j)) - \phi(\load_{j-1}) \leq \phi(\load_{j-1} + x_j(c)) - \phi(\load_{j-1})$ for all configurations~$c \in [q_j]$. As~$\sum_{c=1}^{q_j} y_{cj} = 1$ by feasibility of~$(y_{cj})$, this implies
    \begin{equation}\label{eq_greedy_increase}
        \phi(\load_{j-1} + x_j(c_j)) - \phi(\load_{j-1}) \leq \sum_{c=1}^{q_j} y_{c_j} \phi(\load_{j-1} + x_{j}(c)) - \phi(\load_{j-1}). 
    \end{equation}

    For simplicity, let~$x_{j}$ denote the load vector of configuration~$c_j$. Further, let~$\load_0 = 0 \in \RR^m$ be the all-zero vector. We can now bound the increase in potential incurred by \Cref{alg_on_config} as follows: 
    \begin{align*}
        \phi(\load_n) - \phi(\load_0) 
        & = \sum_{j=1}^n \sum_{i=1}^m \frac32^{\load_{ij-1}/\lambda} \Big( \frac32^{x_{ij}/\lambda} - 1 \Big) \\ 
        & \leq \sum_{j=1}^n \sum_{c=1}^{q_j} y_{c_j} 
            \sum_{i=1}^m  \frac32^{\load_{ij-1}/\lambda} \Big( \frac32^{x_{ij}(c)/\lambda} - 1 \Big) \\ 
       &  \leq 
       \sum_{i=1}^m \frac32^{\load_{in}/\lambda} \sum_{j=1}^n \sum_{c=1}^{q_j} y_{c_j} \Big( \frac32^{x_{ij}(c)/\lambda} -1 \Big), 
   \intertext{where the first inequality holds due to~\eqref{eq_greedy_increase}, and the second inequality holds because the load on machine~$i$ only increases over time. 
       Using a simple algebraic computation, we can bound $\frac32^z - 1 \leq \frac12 z$ for~$z \in [0,1]$. As~$y_{c_j}$ is feasible, we know that~$x_{ij}(c) \leq \lambda$ for all~$c$ with~$y_{c_j} > 0$. Hence, }
        \phi(\load_n) - \phi(\load_0)  & \leq \sum_{i=1}^m \frac32^{\load_{in}/\lambda} \sum_{j=1}^n \sum_{c=1}^{q_j} y_{c_j} \frac{x_{ij}(c)}{2\lambda}
        \intertext{Using again that~$y_{c_j}$ is feasible and satisfies $\sum_{j=1}^n \sum_{c=1}^{q_j} x_{ij}(c) \cdot y_{c_j}  \leq \lambda$ for all resources~$i \in [m]$, we get} 
        \phi(\load_n) - \phi(\load_0) & \leq \frac12 \sum_{i=1}^m \frac32^{\load_{in}/\lambda} = \frac12 \phi(\load_n) 
   \end{align*}
    After rearranging, we get $\phi(\load_n) \leq 2 \phi(\load_0) = 2m$ by choice of~$\load_0$. Taking logarithms and using that~$\log_{3/2}(z)$ is monotonically increasing, we conclude the proof with 
    \begin{equation*}
        \max_{1 \leq i \leq m} \load_{in} \leq \log_{3/2} (2m) \lambda.
    \end{equation*}
\end{proof}



%-------------------------------------------------------------------------------------------
\subsection{Online Stochastic Configuration Balancing}

The goal of this section is to extend \Cref{thm_dcb_on} to stochastic requests. Recall that by \ref{thm_adap_restart}, the random variables can be split into a truncated and an exceptional part without increasing \Opt{} by more than a constant factor. 

The main ingredient for generalizing \Cref{thm_dcb_on} to the stochastic setting is to treat the exceptional parts of a requests's configuration as a \emph{resource requirement} for an additional, artificial resource indexed by~$0$. The second ingredient is again a strong lower bound on the maximum of sums of independent, bounded random variables; similar to \Cref{lem_max_bound_logm}. 

Let~$\lambda$ denote the current guess of the optimum as required by \Cref{lem_guess_and_double}, and let~$\tau = 2 \lambda$ be the truncation threshold. Given a request~$j$ and one of its configurations~$c \in [q_j]$, let~$x_{0j}(c) := \EE[\max_{1\leq i \leq m} X_{ij}^E(c)]$ and~$x_{ij}(c) := \EE[X_{ij}^T(c)]$. We interpret~$x(c) \in \RR_{\geq 0}^{m+1}$,~$c \in [q_j]$ as input to (deterministic) online configuration balancing with~$m+1$ resources. We summarize the algorithm below.

\begin{algorithm}
    \DontPrintSemicolon
    \caption{Online Configuration Balancing with Stochastic Requests}
    \label{alg_on_stoch_config}  
    \textbf{upon arrival of request $j$}\;
    $x_{0j}(c) \leftarrow \EE[\max_i X_{ij}^E(c)]$ for all $1 \leq c \leq [q_j]$\;
    $x_{ij}(c) \leftarrow \EE[X_{ij}^T(c)]$ for all $c \in [q_j]$ and $i \in [m]$\;
    run \Cref{alg_on_config} for configuration vector~$x_j(c)$ with resources $0,\ldots, m$
\end{algorithm}

For the analysis of the algorithm, we use again the linear program~\eqref{eq_lpstochconfig}. With the above definition of $x_{ij}(c)$ for~$j \in [n]$,~$c \in [q_j]$, and~$0 \leq i \leq m$ used by \Cref{alg_on_stoch_config}, this LP is equivalent to~\eqref{eq_lpconfig}. Hence, \Cref{thm_dcb_on} immediately guarantees $\sum_{j=1}^n \EE[X_{ij}^T(c_j)] \leq O(\log m) \lambda$ for all resources~$i\in [m]$ as well as 
$\sum_{j=1}^n \EE[\max_i X_{ij}^E(c_j)] \cdot y_{cj} \leq O(\log m) \lambda$ 
if~\eqref{eq_lpstochconfig} is feasible for~$\lambda$. In order to extend this to a bound on the maximum load incurred by~\Cref{alg_on_stoch_config}, we need the following bound on the maximum of sums of bounded random variables. 

\begin{lem}\label{lem_max_bound_logm}
    Let~$S_1, \ldots, S_m$ be sums of independent random variables bounded in~$[0,\tau]$ such that~$\EE[S_i] \leq O(\log m) \tau$ for all~$1 \leq i \leq m$. Then,~$\EE[\max_i S_i] \leq O(\log m) \tau$. 
\end{lem}

\begin{proof}
    Let~$C \in \RR$ be a constant such that~$\EE[S_i] \leq C \tau \log m$ for all~$1 \leq i \leq m$ and fix~$t > 2e C \tau \log m$, where~$e$ is the Euler constant. Fixing~$i\in[m]$, we know that the random variables constituting~$S_i$ are independent and bounded by~$\tau$. Hence, using the third Chernoff-Hoeffding bound in \Cref{lem_chernoff}, we have~$\PP[S_ i > t] < 2^{-t}$. Therefore, 
    \begin{align*}
        \EE\Big[ \max_{1 \leq i \leq m} S_i \Big] \notag
        & = \int_{0}^\infty \PP\Big[ \max_{1 \leq i \leq m} S_i  > t  \Big] dt \\
        & \leq O(\log m)\tau + \int_{2eC \tau \log m}^\infty  \PP\Big[ \max_{1 \leq i \leq m} S_i  > t  \Big] dt \\
        & \leq O(\log m)\tau + \sum_{i=1}^m \int_{2eC \tau \log m}^\infty \PP\Big[ S_i  > t  \Big] dt \\
        & \leq O(\log m)\tau + m \int_{2 e C \tau \log m}^\infty 2^{-t} dt \\
        & = O(\log m) \tau, 
    \end{align*}
    where the third line uses a union bound over all~$i \in [m]$. 
    
    Note that the proof only requires that the random variables contributing to~$S_i$ for a fixed~$i$ are independent, but it is not necessary that the~$S_i$ are independent from each other. 
\end{proof}

We are now ready to prove the main result of this section, the following theorem. 

\begin{theorem}\label{thm_cb_on}
    If \eqref{eq_lpstochconfig} is feasible for~$\lambda > 0$, then \Cref{alg_on_stoch_config} achieves a maximum load of~$O(\log m)\lambda$. 
\end{theorem}

\begin{proof}
    As before, let~$c_j$ denote the configuration selected by~\Cref{alg_on_stoch_config} for request~$j$. Then, 
    \[
        \EE \Big[\max_{i \in [m]} \sum_{j=1}^n X_{ij}(c_j) \Big] \leq \EE \Big[\max_{i \in [m]} \sum_{j=1}^n X_{ij}^T(c_j) \Big] + \EE \Big[\max_{i \in [m]} \sum_{j=1}^n X_{ij}^E(c_j) \Big]. 
    \]
    Hence, it is sufficient to bound the exceptional and the truncated parts separately. The correct bound on the truncated parts follows immediately from the fact that~\Cref{thm_dcb_on} guarantees~$\sum_{j=1}^n \EE[X_{ij}^T(c_j)] \leq O(\log m) \lambda$ for all~$i \in [m]$ and \Cref{lem_max_bound_logm}. 
    For the exceptional parts, we observe that 
    \[
        \EE\Big[\max_{i \in [m]} \sum_{j=1}^n X_{ij}^E(c_j) \Big] \leq 
        \EE\Big[\sum_{j=1}^n \max_{i \in [m]} X_{ij}^E(c_j) \Big] \leq O(\log m) \lambda,
    \]
    where the second inequality follows again from~\Cref{thm_dcb_on}. 
\end{proof}

==> old_unrelated+routing.tex <==
\section{Unrelated Load Balancing and Virtual Circuit Routing}
In this section, we build on our results for configuration balancing and apply them to stochastic load balancing on unrelated machines as well as stochastic virtual circuit routing.  

\subsection{Scheduling}
Recall that load balancing on unrelated machines is a special case of configuration balancing: Creating one configuration for every machine choice job~$j$ has, we can easily reduce the former problem to the latter. Hence, we can split the random processing times into their truncated and exceptional parts and use \Cref{thm_adap_restart}: For any fixed truncation threshold~$\tau \geq 2 \EE[\Opt]$, there exists an adaptive policy with expected makespan and total expected exceptional load at most~$2 \EE[\Opt]$. 

%Thus, we directly combine the reduction of load balancing to configuration balancing with the reduction of stochastic requests on~$m$ resources to deterministic requests on~$m+1$ resources: For a job~$j$, let~$X_{ij}$ denote its (random) processing time if assigned to machine~$i$. We set 

%\begin{equation*}
%    x_{ij}(c) = 
%    \begin{cases}\EE \big [X_{cj} \cdot \one_{X_{cj} \geq \tau}\big] = \EE \big [X_{cj}^E \big] & \textup{ if } i = 0 \\ 
%        \EE \big [X_{cj} \cdot \one_{X_{cj} < \tau}\big] = \EE \big [X_{cj}^T \big] & \textup{ if } i = c \\ 
%        0 & \textup{ otherwise.}
%    \end{cases}
%\end{equation*} 

\subsubsection{Offline scheduling} 
For offline stochastic load balancing, we observe that \eqref{eq_lpstochconfig}  is equivalent to the following generalized assignment LP:  
    \begin{equation}\tag{$\lpsched$}\label{eq_lpsched}
       \begin{array}{rll}
         \sum_{ij} \mathbb{E} [X_{ij}^E] \cdot y_{ij} & \leq \tau \\
         \sum_j \mathbb{E} [X_{ij}^T] \cdot y_{ij} & \leq \tau &\quad\forall i\\
         \sum_i y_{ij} &  = 1 &\quad\forall j\\
         y_{ij} & \geq 0 &\quad\forall i,j
        \end{array} 
    \end{equation}
Given a feasible solution to \eqref{eq_lpsched}, we use the well-known rounding algorithm by Shmoys and Tardos \cite{DBLP:journals/mp/ShmoysT93} to obtain an integral assignment of jobs to machines. We summarize this algorithm below. 

\begin{algorithm}
    \DontPrintSemicolon
    \caption{Offline Stochastic Load Balancing}
    \label{alg_off_stoch_sched} 
    solve \eqref{eq_lpsched} \;
    use Shmoys-Tardos to obain an integral assignment
\end{algorithm}

Having this algorithm at hand, we are now ready to prove \Cref{thm_unrel_lb_off}. 

\begin{proof}[Proof of \Cref{thm_unrel_lb_off}]
    We note that the LP used by Shmoys and Tardos also includes pruning constraints of the form $y_{ij} = 0$ for $i$ and~$j$ with $\mathbb{E} [X_{ij}^T] > \tau$. But by definition of truncated parts, we have $\mathbb{E} [X_{ij}^T] < \tau$. Thus, the pruning constraints are unnecessary. Hence, we can indeed use the efficient algorithm by Shmoys and Tardos to obtain an integral solution with only a small additive violation in the second constraint~\cite{DBLP:journals/mp/ShmoysT93}. 
    
    Thus, if \eqref{eq_lpsched} is feasible, then we can obtain an integral solution, i.e., a non-adaptive policy, whose expected truncated load is $O(\tau)$ per machine and total expected exceptional load is at most $\tau$. To show feasibility, we consider the adaptive policy guaranteed by \Cref{thm_adap_restart}, and let the events~$j \rightarrow i$ be with respect to this policy. We use the natural setting of the $y$-variables given this policy: for all~$i,j$, we take~$y_{ij} = \PP(j \rightarrow i)$. It is clear that $\sum_i y_{ij} = 1$ for all $j$ and $0 \leq y_{ij} \leq 1$ for all $i,j$. It remains to verify the exceptional- and truncated load constraints. For the former we observe 
    \[
        \sum_{ij} \mathbb{E}[X_{ij}^E] \cdot y_{ij} = \sum_{ij} \mathbb{E}[X_{ij}^E \cdot \one_{j \rightarrow i}] \leq 2 \cdot \mathbb{E}[\Opt] \leq \tau,
    \]
    where in the first step we use the fact that the decision to schedule job $j$ on machine $i$ is independent of its realization, and in the second we use the properties of the policy. Similarly, for the truncated constraint for each $i$:
    \[
        \sum_{j} \mathbb{E}[X_{ij}^T] \cdot y_{ij} = \sum_{j} \mathbb{E}[X_{ij}^T \cdot \one_{j \rightarrow i}] \leq 2 \cdot \mathbb{E}[\Opt] \leq \tau.
    \]
    Hence, \Cref{lem_max_bound_logm} guarantees that the expected makespan of the schedule returned by our algorithm is bounded by $O\big(\frac{\log m}{\log \log m}\big) \Opt$.
\end{proof}

\subsubsection{Online scheduling} For online load balancing on~$m$ machines, we directly reduce the problem to online configuration balancing with~$m$ resources by using creating~$m$ configurations for job~$j$, one for every machine that job~$j$ can be assigned to. In other words, we set
\begin{equation*}
    X_{ij}(c) = 
    \begin{cases} 
        X_{cj}  & \textup{ if } i = c \\ 
        0 & \textup{ otherwise}
    \end{cases}
\end{equation*}
and run \Cref{alg_off_config_stoch}. 


\begin{proof}[Proof of \Cref{thm_unrel_lb_on}] 
    Since every job has at most~$m$ configurations associated, the configuration~$c_j$, that minimizes the increase in the potential function in Line~\ref{alg_on_config_argmin}, can be found efficiently. Hence, \Cref{{lem_on_config_runtime}} guarantees that \Cref{alg_off_config_stoch} runs in polynomial time. Thus, the proof follows directly from \Cref{thm_cb_on}.
\end{proof}



\subsection{Routing}

Virtual circuit routing is another special case of configuration balancing: Given any instance of the former, which consists of a directed graph with $m$ edges and $n$ source-sink pairs, the resulting configuration balancing instance has $m$ resources, one for each edge, and $n$ requests, one for each source-sink pair, such that there is one configuration per source-sink path in the graph.

Note that unlike load balancing, where a request has at most $m$ configurations, for routing, a request can have exponentially many configurations. Thus, to obtain polynomial-time algorithms for routing, we cannot explicitly represent all configurations. In particular, to prove \Cref{thm_route_off}, we need to show how to solve \eqref{eq_lpstochconfig} efficiently in the special case of routing, and to prove \Cref{thm_route_on}, we need to show how to find the configuration (i.e. the path) that minimizes the increase in the potential $\Phi$. \fra{I changed the order slightly and created some lemmas and proofs along the way.}

\subsubsection{Offline routing: solving \eqref{eq_lpstochconfig}}

We first re-write \eqref{eq_lpstochconfig} for the special case of routing. For a request $j$, let $\mathcal P_j$ be the collection of all $s_j$-$t_j$ paths in the input graph $G = (V,E)$. For each request~$j$ and path~$P \in \mathcal P_j$, the variable~$y_{Pj}$ denotes the decision to route request~$j$ along path $P$. Thus, we want to solve the following ``path assignment'' LP. 
\rud{I removed the pruning constraint because I don't think we use it anywhere and it's easier to take the dual this way. Do we use it for the potential function at all? Franziska can you confirm?}
\fra{my concern is that the classical LP needs the pruning constraints and we don't have a proof that the integrality gap is indeed bounded in our case ... }
\fra{Thinking about this, we can easily change the definition of~$\mathcal P_j$ such that any path with an edge~$e$ with~$\EE[X_{ej}] > \tau$ is not contained in the set. We slightly adapt the algorithm such that those edges are removed from the graph and not considered as~$\bar e$ at all.}
\begin{equation}\tag{$\lppath$}\label{eq_lppath}
	\begin{array}{rll}
		\sum_{P \in P_j} y_{Pj} &  = 1 &\quad\forall~j\in[n] \\
		\sum_{j=1}^n \sum_{P \in P_j} \EE[X_{ej}^T] \cdot y_{Pj}  &  \leq \tau &\quad\forall~e \in E \\
		\sum_{j=1}^n \sum_{P \in P_j} \EE[\max_{e \in P} X_{ej}^E] \cdot y_{Pj} & \leq \gamma \\
		y_{Pj} & \geq 0 & \quad \forall~j\in[n], ~P \in P_j 
	\end{array} 
\end{equation}

Note that \eqref{eq_lppath} has an exponential number of variables. For classical congestion minimization problems, the path-assignment LP formulation is equivalent to a flow formulation \addref, which can be solved optimally in polynomial time using results about flows in networks. In our case, however, we additionally have the third constraint in the LP, which does not allow for a straight-forward equivalent flow formulation. Therefore, we use LP duality in order to solve it efficiently: More precisely, we give a separation oracle for its dual LP and apply complementary slackness. \rud{is there a black box way to do this (i.e. if you can separate dual, then you can optimize primal?}\fra{I think so, although I don't have a good reference for it}\addref For obtaining the dual, we add the trivial objective to maximize $0^T y$ to \eqref{eq_lppath}. Hence, the dual of $\lppath$ is given by the following LP. %has variables $a_j$ for all $j \in [n]$, $b_e$ for all $e \in E$ and $c$ for the three types of constraints of \eqref{eq_lppath}, respectively:

\begin{equation}\tag{$\lppathd$}\label{eq_lppathd}
	\begin{array}{rll}
	    \min \sum_j a_j + \sum_e b_e \cdot \gamma + c \cdot \tau &\\
		s.t. \quad a_j + \sum_{e \in P} b_e \cdot \EE[X_{ej}^T] + c \cdot \EE[\max_{e \in P} X_{ej}^T] & \geq 0 & \quad\forall j \in [n], ~P \in\mathcal P_j\\
		b_e & \geq 0 &\quad\forall~e \in E \\
		c & \geq 0
	\end{array} 
\end{equation}

For solving \eqref{eq_lppathd}, consider a request~$j$ and a path~$P \in \mathcal P_j$. The expected exceptional part of routing~$j$ along~$P$ is $\EE \big[\max_{e \in P} X_{ej} ^E \big] =  \max_{e \in P} \EE \big[\big({X_j}/{c_e}\big)^E\big]$, which is the expected exceptional part of the smallest-capacity edge~$\bar e_j$ along the path. Given this edge~$\bar e_j$, a particular choice of the dual variables is feasible for the first constraint of \eqref{eq_lppathd} if and only if
\[\min_{P \in \mathcal P_j \, : \, \min_{e \in P} c_e \geq c_{\bar e_j} } \bigg( \sum_{e \in P} b_e \cdot \EE\big[X_{ej}^T\big] + c \cdot \EE\big[\max_{e \in P} X_{ej}^T\big] \bigg) \geq -a_j \quad\forall~ j.\] 
Hence, for each request~$j$, it remains to find a path~$P \in \mathcal P_j$ that is minimal w.r.t. $b_e \cdot \mathbb{E}[X_{ej}^T]$. By letting every edge~$\bar e$ be the smallest-capacity edge and removing any smaller-capacity edges from the graph, this becomes a shortest~$s_j$-$t_j$ path problem. We summarize the resulting separation oracle in \Cref{alg_route_off}. 

\begin{algorithm}
    \DontPrintSemicolon
    \caption{Separation oracle for \eqref{eq_lppathd}}
    \label{alg_route_off} 
    $(a,b,c) \leftarrow$ current solution of \eqref{eq_lppathd} \;
    \uIf{$b_e < 0$ for some $e \in E$ {\normalfont \bfseries or }$c < 0$} {
        return the violated non-negativity constraint\;
    }
    \Else{
        \For{$j$ {\normalfont \bfseries and }edge $\bar{e} \in E$}{
            $E_{\bar e}\leftarrow \{e \in E: c_e \geq  c_{\bar{e}} \}$ \;
            $G_{\bar{e}} \leftarrow$ $(V, E_{\bar e}) $ \;
            $P_{j\bar e} \leftarrow$ shortest $s_j$-$t_j$ path in $G_{\bar{e}}$ w.r.t. $b_e \cdot \mathbb{E}[X_{ej}^T]$ \;
            \If{$\sum_{e \in P_{j\bar{e}}} b_e \cdot \EE[X_{ej}^T] + c \cdot \EE[\max_{e \in P_{j\bar{e}}} X_{ej}^T] < - a_j$} {
                return $\sum_{e \in P_{j\bar{e}}} b_e \cdot \EE[X_{ej}^T] + c \cdot \EE[\max_{e \in P_{j\bar{e}}} X_{ej}^T] \geq - a_j$\;
            }
%            \Else {
%               continue\;
%            }
        }
        return ``feasible''\;
    }
\end{algorithm}

Given a feasible solution to~\eqref{eq_lppath}, we run \Cref{alg_off_config_stoch} on the configuration-balancing instance obtained from the offline routing instance. 


\begin{lem}\label{lem_routing_dual}
    \Cref{alg_route_off} solves \eqref{eq_lppathd} optimally in polynomial time. 
\end{lem}

\begin{proof}
    Since shortest paths can be found in polynomial time\addref, \Cref{alg_route_off} indeed runs in polynomial time. Further, if there is a~$e \in E$ with~$b_e < 0$ or if~$c<0$, then \Cref{alg_route_off} correctly outputs the violated constraint. 
    
    It remains to consider the case when~$b, c \geq 0$. In this case, it remains to show for each request~$j$ that we find some $\bar{e} \in E$ such that $P_{j \bar{e}}$ achieves the minimum $\min_{P \in P_j} \big( \sum_{e \in P} b_e \cdot \EE[X_{ej}^T] + c \cdot \EE[\max_{e \in P} X_{ej}^T] \big)$. 
    
    Consider any request $j$ such that the minimum is achieved by some $s_j$-$t_j$ path $P^*$. Let $e^*$ be the smallest-capacity edge along $P^*$. We claim for the correct guess $\bar{e} = e^*$, $P_{j \bar{e}}$ achieves the minimum. To see this, observe that $P^*$ is a $s_j$-$t_j$ path in the graph $G_{\bar{e}}$, so the algorithm will choose $P_{j \bar{e}}$ with $\sum_{e \in P_{j\bar{e}}} b_e \cdot \EE[X_{ej}^T] \leq \sum_{e \in P^*} b_e \cdot \EE[X_{ej}^T]$ by definition of the edge weights. Further, we have $c \cdot \EE[\max_{e \in P_{j\bar{e}}} X_{ej}^T] \leq c \cdot \EE[\max_{e \in P^*} X_{ej}^T]$, because the latter maximum is achieved by edge $\bar{e}$, and by definition of the residual graph, $P_{j \bar{e}}$ cannot use any edges with smaller capacity than $\bar{e}$. Combining these two bounds shows that $P_{j \bar{e}}$ achieves the minimum. This in turn implies that \Cref{alg_route_off} returns a constraint violated by~$(a,b,c)$ if such a constraint exists. 
\end{proof}



\begin{proof}[Proof of \Cref{thm_route_off}] 
    \Cref{lem_routing_dual} guarantees that \eqref{eq_lppath} can be solved optimally in polynomial time. Hence, \Cref{lem_off_config_stoch} implies that \Cref{alg_off_config_stoch} runs in polynomial time and achieves a maximum congestion of $O\big(\frac{\log m}{\log \log m}\big) \Opt$. 
\end{proof}


% Consider a request $j$ and fixed path $P \in P_j$. The expected exceptional part of the configuration corresponding to choosing this request is exactly $\EE \big[\max_{e \in P} X_{ej} ^E \big] =  \max_{e \in P} \EE \big[\big({X_j}/{c_e}\big)^E\big]$, which is the expected exceptional part of the smallest capacity edge along the path. Further, note that a setting of the dual variables satisfies the first constraint of $\lppathd$ if and only if:
%\[\min_{P \in P_j} \big( \sum_{e \in P} b_e \cdot \EE[X_{ej}^T] + c \cdot \EE[\max_{e \in P} X_{ej}^T] \big) \geq -a_j \quad\forall~ j.\]
% We can find the path achieving this minimum by guessing the smallest capacity edge used by the optimal path and solving a shortest $s-t$ path problem on an appropriate residual graph.



%It is clear that \Cref{alg_route_off} is efficient. If some $b_e$ or $c$ is negative, then it is clear that the algorithm correctly separates the given solution from $\lppath$. It remains to consider the case where $b, c \geq 0$. In this case, it suffices to show for every request $j$ that we find some $\bar{e} \in E$ such that $P_{j \bar{e}}$ achieves the minimum $\min_{P \in P_j} \big( \sum_{e \in P} b_e \cdot \EE[X_{ej}^T] + c \cdot \EE[\max_{e \in P} X_{ej}^T] \big)$.

%Consider any request $j$ such that the minimum is achieved by some $s_j-t_j$ path $P^*$. Let $e^*$ be the smallest capacity edge along $P^*$. We claim for the correct guess $\bar{e} = e^*$, $P_{j \bar{e}}$ achieves the minimum. To see this, observe that $P^*$ is a $s_j-t_j$ path in the residual graph $G_{\bar{e}}$, so the algorithm will choose $P_{j \bar{e}}$ with $\sum_{e \in P_{j\bar{e}}} b_e \cdot \EE[X_{ej}^T] \geq \sum_{e \in P^*} b_e \cdot \EE[X_{ej}^T]$ by definition of the edge weights. Further, we have $c \cdot \EE[\max_{e \in P_{j\bar{e}}} X_{ej}^T] \leq c \cdot \EE[\max_{e \in P^*} X_{ej}^T]$, because the latter maximum is achieved by edge $\bar{e}$, and by definition of the residual graph, $P_{j \bar{e}}$ cannot use any edges with smaller capacity than $\bar{e}$. Combining these two bounds shows that $P_{j \bar{e}}$ achieves the minimum..

\subsubsection{Online routing: minimizing increase in $\Phi$}

For online virtual circuit routing, we assume that a  sequence of source sink-pairs $(s_j,t_j)$ for $j = 1, \dots, n$ arrive online. To implement \Cref{alg_on_stoch_config} efficiently, given a load vector $\load = (\load_0, \dots, \load_m)$ and source-sink pair $(s,t)$ with random demand $X \geq 0$, we need to choose a $s$-$t$ path in $G$ that minimizes the increase in $\Phi$ with respect to some fixed truncation threshold $\tau$. Recall that we index the edges of $G$ by $1, \dots m$, while $L_0$ is the load of an additional, artificial resource that captures the total expected exceptional load.

As in the offline setting, the expected exceptional part of the configuration corresponding to choosing a particular~$s_j$-$t_j$ path is the expected exceptional part of the smallest-capacity edge along the path. Thus, the increase in potential due to choosing a path~$P$ is\rud{not exactly right; need to put capacities before the truncation; to fix}
\[
    \big( (3/2)^{ (\load_{0} + ( \max_{e \in P} \frac{1}{c_e} ) \EE [X_j^E]) / \tau    } - (3/2)^{ \load_{0}  / \tau    }\big) + 
    \sum_{e \in P}  \big( (3/2)^{ ( \load_{e} + \frac{1}{c_e}\EE[X_j^T])    / \tau } - (3/2)^{  \load_{e}    / \tau }\big).
\]
The first term is the increase due to the exceptional part (the smallest-capacity edge along $P$), and the remaining terms are the per-edge contributions due to the truncated parts. Analogously to the previous section, we guess the smallest-capacity edge, and solve a shortest $s_j$-$t_j$ path problem to find the minimizing path. This is summarized in \Cref{alg_route_on}. 

\begin{algorithm}
    \DontPrintSemicolon
    \caption{Minimizing increase in $\Phi$ for virtual circuit routing}
    \label{alg_route_on} 
    $L\leftarrow$ current load vector \;
%    $s_j, t_j, X$ with demand $X$ \;
    \For{$\bar{e} \in E$}{
        $E_{\bar e}\leftarrow \{e \in E: c_e \geq  c_{\bar{e}} \}$ \;
        $G_{\bar{e}} \leftarrow$ $(V, E_{\bar e}) $ \;
        $P_{j\bar e} \leftarrow$ shortest $s_j$-$t_j$ path in $G_{\bar{e}}$ w.r.t. $\big( (3/2)^{ ( \load_{e} + \frac{1}{c_e}\EE[X^T])    / \tau } - (3/2)^{  \load_{e}    / \tau }\big)$ \;
%         Construct the \textit{residual graph} $G_{\bar{e}}$ from $G$ by deleting all edges with capacities strictly smaller than $c_{\bar{e}}$ \;
%        Find the shortest $s-t$ path in $G_{\bar{e}}$ with respect to edge weights $\big( (3/2)^{ ( \load_{e} + \frac{1}{c_e}\EE[X^T])    / \tau } - (3/2)^{  \load_{e}    / \tau }\big)$ for each edge $e$ of $G_{\bar{e}}$.\;
%        Let $P_{\bar{e}}$ be the resulting path (if such a path exists)\;
    }
    $P_{j} \leftarrow \arg \min_{P_{j\bar e}}$ increase in $\Phi$ \;
\end{algorithm}

Given this subroutine for finding the minimizing path~$P_j$, which uniquely corresponds to the configuration~$c_{P_j}$, we can run \Cref{alg_on_stoch_config} to solve online virtual circuit routing. For analyzing its running time, we need the following lemma. 

\begin{lem}\label{lem_route_minincrease}
    Given a request~$j$, \Cref{alg_route_on} efficiently returns a path~$P_j$ that minimizes the increase in~$\Phi$. 
\end{lem}

\begin{proof}
    It is clear that \Cref{alg_route_on} is efficient. To see that it also finds a path that minimizes the increase in $\Phi$, let $P_j^*$ be such an optimal path with smallest-capacity edge~$e^*$. For the correct guess~$\bar{e} = e^*$,~$P_j^*$ is a $s_j$-$t_j$ path in the graph~$G_{\bar e}$. Thus, \Cref{alg_route_on} chooses $P_{j\bar e}$ such that the per-edge contributions due to the truncated parts of $P_{j\bar e}$ are at most those due to $P_j^*$ by definition of the edge weights. Further, the exceptional part of $P_{j\bar e}$ is at most that of $P_j^*$, because $P_{j \bar e}$ does not use any edges with capacity smaller than~$c_{\bar e}$ by definition of the graph~$G_{\bar e}$. We conclude that $P_{j\bar e}$ is also a shortest~$s_j$-$t_j$ path. 
\end{proof}


\begin{proof}[Proof of \Cref{thm_route_on}]
    \Cref{lem_route_minincrease} guarantees that for each request~$j$ a path~$P_j$ that minimizes the increase in the potential function~$\Phi$ can be found in polynomial time. As any~$s_j$-$t_j$ path corresponds to a unique configuration for request~$j$, \Cref{lem_on_config_runtime} implies that \Cref{alg_on_stoch_config} runs in polynomial time while \Cref{thm_cb_on} implies that the chosen paths incur an expected maximum congestion of at most~$O(\log m)\Opt$. 
\end{proof}

==> savedText.tex <==
Let us define a common generalization: the \emph{configuration
  balancing} has~$m$ resources and~$n$ requests. Every request~$j$
has~$q_j$ possible configurations~$x_j(1), \ldots, x_j(q_j) \in
\RR_{\geq 0}^m$. We must choose one configuration~$c_j \in [q_j]$ per
request, which adds $x_j(c_j)$ to the load vector on the resources.
% , i.e., load~$x_{ij}(c)$ is added to resource~$i$ for~$i\in [m]$.
The goal is to % choose a configuration for each request to 
minimize the makespan, i.e., theload of the most-loaded resource.  % We call this maximum load the makespan. Load balancing and virtual circuit routing are both special cases of 
Configuration balancing generalizes both the examples above, by taking
the $m$ resources to be the $m$ machines or edges respectively;  % and defining the
each configurations now corresponds to assigning a job to some machine
or routing a request along a particular source-sink
path. \fra{explicit vs. implicit} 








theorem 1.1 and 2.2:

 \fnew{When the configurations are given explicitly,} there is an efficient randomized \emph{offline} algorithm \nnew{that computes a non-adaptive policy} for configuration balancing with stochastic requests that $\Theta\big(\frac{\log m}{\log \log m}\big)$-approximates the optimal offline adaptive policy.  There exists an online algorithm for configuration balancing with stochastic requests that~$O(\log m)$-approximates 
    %is~$O(\log m)$-competitive relative to 
    the optimal adaptive offline policy. 
    
    
    
    
    
    
    
    mplies the following theorem. 

\ag{Combine the following pairs of theorems into one each?}
\begin{theorem}\{thm_unrel_lb_off}
	There exists an efficient deterministic algorithm that computes a non-adaptive policy for load balancing on unrelated machines with stochastic jobs that $O\big(\frac{\log m}{\log \log m}\big)$-approximates the optimal adaptive policy.
\end{theorem}

This result is asymptotically tight as shown by the lower bound of~$\Omega\big(\frac{\log m}{\log \log m}\big)$ on the adaptivity gap by~\cite{DBLP:journals/mor/Gupta0NS21}. In particular, this implies that the adaptivity gap for stochastic load balancing is $\Theta\big(\frac{\log m}{\log \log m}\big)$. 

For online load balancing, there is a lower bound of~$\Omega(\log m)$ on the competitive ratio of any deterministic algorithm, even for deterministic requests~\cite{DBLP:journals/jal/AzarNR95}. We show a matching (up to constants) upper bound.  

\begin{theorem}\label{thm_unrel_lb_on}
	There exists an efficient online algorithm that computes a non-adaptive policy for load balancing on unrelated machines with stochastic jobs that $O(\log m)$-approximates the optimal adaptive policy.
\end{theorem}





\begin{theorem}\label{thm_route_off}
    There exists an efficient randomized offline algorithm that computes a non-adaptive policy for routing with stochastic requests that $O\big(\frac{\log m}{\log \log m}\big)$-approximates the optimal adaptive policy.
\end{theorem}

For online virtual circuit routing, we carefully select a subset of \fnew{polynomially many} configurations that contains the configuration chosen by the greedy algorithm, even when presented with all configurations. Therefore, we can apply \Cref{thm_config_on} to obtain the following theorem. 

\begin{theorem}\label{thm_route_on}
    There exists an efficient  online algorithm that computes a non-adaptive policy for routing with stochastic jobs that $O(\log m)$-approximates the optimal adaptive policy.
\end{theorem}



\begin{theorem}\label{thm_rel_lb_off}
	There exists an efficient offline algorithm that computes an adaptive policy for load balancing on related machines with stochastic jobs that $O(1)$-approximates the optimal  adaptive policy.
\end{theorem}

\begin{theorem}\label{thm_rel_lb_on}
	There exists an efficient online algorithm that computes an adaptive policy for load balancing on related machines with stochastic jobs that $O(\log \log m)$-approximates the optimal adaptive policy.
\end{theorem}
















    \begin{comment}
    \medskip
    \hrule
    \smallskip
    \hrule
    \smallskip
        \begin{OneLiners}
    	    \item[i.] Run policy $\Opt(J)$.
    	    \item[ii.] At the first decision that chooses a configuration, say $c$ of request $j$, that becomes exceptional ($\max_i X_{ij}(c) > \tau$), we stop running $\Opt(J)$ immediately after realizing this request.
    	    %Note that if no decision chooses an exceptional configuration, then we run $\Opt(J)$ to completion, and we are done.
    	    \item[iii.] At the first decision that will choose a configuration, say $c$ of request $j$, with $\EE \big[ \max_i X_{ij}(c) \big] > \tau$ (note we can determine this before actually choosing the configuration), we stop running $\Opt(J)$ before choosing this configuration. 
    	    \item[iv.] Let $R \subset J$ denote the remaining set of unscheduled requests. We have $\lvert R \rvert < \lvert J \rvert$, so let $S(R)$ denote the policy on $R$ guaranteed by \Cref{thm_adap_restart} by induction. Then run policy $S(R)$ to completion.
    	 \end{OneLiners}
     \medskip
     \hrule
     \smallskip
     \hrule
     \medskip
    \end{comment}
